On the Complexity of Intersection Non-emptiness for Star-Free Language Classes

In the Intersection Non-Emptiness problem, we are given a list of finite automata $A_1,A_2,\dots,A_m$ over a common alphabet $\Sigma$ as input, and the goal is to determine whether some string $w\in \Sigma^*$ lies in the intersection of the languages accepted by the automata in the list. We analyze the complexity of the Intersection Non-Emptiness problem under the promise that all input automata accept a language in some level of the dot-depth hierarchy, or some level of the Straubing-Th\'{e}rien hierarchy. Automata accepting languages from the lowest levels of these hierarchies arise naturally in the context of model checking. We identify a dichotomy in the dot-depth hierarchy by showing that the problem is already NP-complete when all input automata accept languages of the levels zero or one half and already PSPACE-hard when all automata accept a language from the level one. Conversely, we identify a tetrachotomy in the Straubing-Th\'{e}rien hierarchy. More precisely, we show that the problem is in AC$^0$ when restricted to level zero; complete for LOGSPACE or NLOGSPACE, depending on the input representation, when restricted to languages in the level one half; NP-complete when the input is given as DFAs accepting a language in from level one or three half; and finally, PSPACE-complete when the input automata accept languages in level two or higher. Moreover, we show that the proof technique used to show containment in NP for DFAs accepting languages in the Straubing-Th\'{e}rien hierarchy levels one ore three half does not generalize to the context of NFAs. To prove this, we identify a family of languages that provide an exponential separation between the state complexity of general NFAs and that of partially ordered NFAs. To the best of our knowledge, this is the first superpolynomial separation between these two models of computation.

==> Definitions.tex <==
\section{A Few Definitions}

\todo[color=gray!10,inline]{HF: Do we want to make $\Sigma$ explicit in the classes themselves? Otherwise, this looks not precise enough.}
In the following, let $\Sigma$ be a finite alphabet.
\paragraph{\bf Polynomial Closure.} For a class of languages~$\mathcal C$,
we denote its closure under finite (possibly empty) union
by~$\FU({\mathcal C})$. Moreover, set
$$
\POL({\mathcal C}):=\FU(\{\,L_0L_1\cdots L_n\mid\mbox{$n\geq 0$ and
  $L_i\in\mathcal C$}\,\})$$ as the polynomial closure of~$\mathcal
C$. Note that $\POL({\mathcal C})$ is exactly the closure of~$\mathcal
C$ under finite (possibly empty) union and finite (non-empty)
concatenation.  Furthermore, $\mathcal C$ is a subset of the
polynomial closure of~$\mathcal C$.

\paragraph{\bf Boolean Operations.} For a class~$\mathcal C$\todo{HF added $\Sigma^+$ in the def. below, as it is not clear if other choices would be allowed} of
languages, we denote by \[\co{\mathcal C} = \{\,\Sigma^+\setminus L\mid
L\in {\mathcal C}, L\subseteq\Sigma^+\,\}\] the set of complements with respect
  to~$\Sigma^+$. For a second closure operation, we consider Boolean
  operations. We denote the Boolean closure of a class~$\mathcal C$ of
  languages of~$\Sigma^+$ by $\BC({\mathcal C})$ (taking complements with
  respect to~$\Sigma^+$).

\paragraph{\bf Dot-depth Hierarchy.} The classes of the dot-depth
hierarchy (DDH) are defined as\todo{HF: Also in this def., it is (formally) not clear if $\Sigma$ is fixed beforehand.}
\begin{align*}
\dd{1/2} & = \POL(\{\,\{w\}\mid w\in \Sigma^+ \}\cup\{\Sigma^+\}), & \\
\dd{n+1} & = \BC(\dd{n+1/2}) & \mbox{for $n\geq 0$,}\\
\noalign{\hbox{and}}
\dd{n+3/2} & = \POL(\dd{n+1}) & \mbox{for $n\geq 0$.}\\
\end{align*}
One can also define $\dd{0}$ as the class that contains all finite and co-finite languages.

\paragraph{\bf Straubing-Th{\'e}rien Hierarchy.} The classes of the Straubing-Th{\'e}rien
hierarchy (STH) are defined as
\begin{align*}
\st{1/2} & = \POL(\{\,\Sigma^*a\Sigma^*\mid a\in \Sigma\,\}), & \\
\st{n+1} & = \BC(\st{n+1/2}) & \mbox{for $n\geq 0$,}\\
\noalign{\hbox{and}}
\st{n+3/2} & = \POL(\st{n+1}) & \mbox{for $n\geq 0$.}\\
\end{align*}
One can also define $\st{0}$ as the class that contains the
emptyset~$\emptyset$ and~$\Sigma^+$.

\paragraph{\bf Inclusion Relations.} The following inclusion relations in
each hierarchy are easy to see from the definitions:
\begin{align*}
  \dd{n+1/2}\cup\co\dd{n+1/2} & \subseteq \dd{n+1} \subseteq \dd{n+3/2}\cap\co\dd{n+3/2}\\
  \noalign{\hbox{and}}
  \st{n+1/2}\cup\co\st{n+1/2} & \subseteq \st{n+1} \subseteq \st{n+3/2}\cap\co\st{n+3/2}\\
\end{align*}
for $n\geq 0$.  Comparing these hierarchies with each other by
inclusion we find that it holds that
\begin{enumerate}
\item $\st{n-1/2}\subseteq \dd{n-1/2}\subseteq \st{n+1/2}$,
\item $\co\st{n-1/2}\subseteq \co\dd{n-1/2}\subseteq \co\st{n+1/2}$,
  and
\item $\st{n}\subseteq \dd{n}\subseteq \st{n+1}$,
\end{enumerate}
for $n\geq 1$.

\paragraph{\bf Alternative Polynomial Closures and Complementation.} 
For alternative definitions there are two points to look at. First,
one finds other versions of the polynomial closure operation in the
literature, see, e.g.,~\cite{PiWe97}:
\begin{align*}
 \POLL({\mathcal C}) &= \FU(\{\,L_0a_1L_2\cdots a_nL_n\mid\mbox{$n\geq 0$,\ $L_i\in{\mathcal C}$, and $a_i\in \Sigma$}\,\})\\
\noalign{\hbox{and}}
 \POLB({\mathcal C}) &= \FU(\{\,u_0L_1u_1\cdots L_nu_n\mid\mbox{$n\geq 0$,\ $L_i\in{\mathcal C}$,\ $u_i\in \Sigma^*$, and if $n=0$, then $u_0\neq\lambda$}\,\}).\\
\end{align*}
A second point is that languages may be defined in a way such that
they contain the empty word. This is a crucial point in the theory
of varieties of finite semigroups, see, e.g.,~\cite{Pi95a}.  We refer to
the Boolean closure of a class~$\mathcal C$ of languages of~$\Sigma^*$ by~$\BCs({\mathcal C})$ (here taking complements with respect
to~$\Sigma^*$). Moreover, let $$\cos{\mathcal C} =\{\, \Sigma^*\setminus L\mid
L\in{\mathcal C}\,\}$$ refer to the set of complements with respect
to~$\Sigma^*$.

\paragraph{\bf Alternative Definitions of DDH and STH.} 
In~\cite{Pi97} one finds the following definition for the levels of
the dot-depth hierarchy. Let $\ddp{1/2}$ be the class of all languages
of~$\Sigma^+$ that can be written as finite unions of languages of the form
$u_0\Sigma^+u_1\cdots \Sigma^+u_m$, where $m\geq 0$ and~$u_i\in \Sigma^*$. For $n\geq
0$, let $\ddp{n+1}=\BC(\ddp{n+1/2})$ and
$\ddp{n+3/2}=\POLB(\ddp{n+1})$.
%
For the Straubing-Th{\'e}rien hierarchy, one finds alternative
definitions in~\cite{St81,Th81}\todo{EA: missing ref}.  Let $\sts{1/2}$ be the class of all
languages of~$\Sigma^*$ that can be written as finite unions of languages
of the form $\Sigma^*a_1\Sigma^*\cdots a_m\Sigma^*$, where $m\geq 0$ and~$a_i\in
\Sigma$. For $n\geq 0$, let $\sts{n+1}=\BCs(\sts{n+1/2})$ and
$\sts{n+3/2}=\POLL(\sts{n+1})$.

It holds that
\begin{enumerate}
\item $\ddp{n/2}=\dd{n/2}$, for $n\geq 1$, \todo{HF: This is only true if $\Sigma$ is fixed.}
\item $\sts{1/2}=\st{1/2}\cup\{\Sigma^*\}$, and
\item $\sts{n/2}=\st{n/2}\cup\{\,L\cup\{\lambda\}\mid L\in\st{n/2}\,\}$.
\end{enumerate}
Thus, the classes $\ddp{n/2}$ and $\dd{n/2}$ coincide, and the
languages in $\sts{n/2}$ are, up to the empty word, the languages in
$\st{n/2}$. For the intersection non-emptiness problem, the slight
difference between $\st{n/2}$ and $\sts{n/2}$ does not make any
difference from the computational complexity point of view.

Let $X$ be a class of automata, we define the $X$ membership problem as follows:
\begin{itemize}
    \item \emph{Input}: Finite automata $A_i=(Q,\Sigma,\delta,q_0,F)$.
\item \emph{Question}: Does $A$ belongs to the class $X$.
\end{itemize}
\todo[inline]{EA: add results with regards to the membership to the level of both hierarchy}

\paragraph{\bf Some Other Important Classes.}
A monoid~$S$ is $\mathcal R$-trivial ($\mathcal L$-trivial, \resp) if,
whenever two monoid elements~$s$ and~$t$ satisfy $sS=tS$ ($Ss=St$,
\resp).
%
{\color{blue} LF: Check, this doesn't look like the right definition to me (instead, should be $sS = tS$ iff $s = t$).}
%
A language accepted by a finite automata is said to be an
$\mathcal R$-trivial ($\mathcal L$-trivial, \resp) language if its
syntactic monoid is $\mathcal R$-trivial ($\mathcal L$-trivial, \resp).
We have the inclusions
$$\sts{1}=\mbox{$\mathcal J$-trivial}\subseteq\left\{
\begin{array}{c}
  \mbox{$\mathcal R$-trivial}\\
  \mbox{$\mathcal L$-trivial}
\end{array}\right\}
\subseteq\sts{3/2}.$$ Here a monoid is $\mathcal J$-trivial if it is
both $\mathcal R$- and $\mathcal L$-trivial. This carries over to
languages accepted by finite automata and their syntactic monoid.

A regular language~$L$ over the alphabet~$\Sigma$ is \emph{piecewise
  testable} if it is the finite Boolean combination of languages of
the form
$$\Sigma^*a_1 \Sigma^*a_2\cdots a_n \Sigma^*,$$
where $a\in \Sigma$ and $n\geq 0$. By definition this is equivalent to the
class $\sts{1/2}$. There is a finer characterization in terms of
$k$-piecewise testable languages, where the scattered words
$a_1a_2\cdots a_n$ are bounded in length by~$k$.\todo{altogether or each of them?}

An $\mathcal R$-expression is a finite union of regular expression of
the form\todo{HF: Why is here $a_2$ not listed but below?} $$\Sigma_0^*a_1\Sigma_1^*\cdots a_m\Sigma_m^*,$$ where $m\geq 0$,
$a_1,a_2,\ldots,a_m\in \Sigma$,\ $\Sigma_i\subseteq \Sigma$, for $0\leq i\leq m$, and
$a_i\not\in \Sigma_{i-1}$, for $1\leq i\leq m$. Then, a language $L$ 
described by an $\mathcal R$-expression is said to be an $\mathcal
R$-expression language.

In~\cite{BMT07} the class of ``alphabetical pattern constraints''
(APC) was introduced.  An APC is a finite union of languages of the
form \[\Sigma_0^*a_1\Sigma_1^*a_2\cdots a_m\Sigma_m^*\] where every~$\Sigma_i$ denotes a
subset of the alphabet~$\Sigma$ and every $a_i\in \Sigma$ denotes a single
letter. Observe the difference in the definition of $\mathcal
R$-expressions and APCs. Hence, APCs corresponds to the set of
expressions defining languages in $\st{3/2}$. The class APC is not
closed under complementation. Consider, e.g., the alphabet $\Sigma=\{a,b\}$
and the APC language $\Sigma^*aa\Sigma^*+\Sigma^*bb\Sigma^*+b\Sigma^*+\Sigma^*a$ and its complement
$(ab)^*$, which is not an APC language. APC are effectively closed
under permutation rewriting, that is, closed under the iterative
application of rules of the form $ab\rightarrow ba$.



\paragraph{\bf Forbidden Pattern Characterizatations.}
At least a few low levels of both hiearchies obey forbidden pattern
characterizations for DFAs, at the moment we think that these
descriptions are not interesting for our research
direction. Nevertheless, let us give two examples:
\begin{enumerate}
\item Let~$M$ be the minimal DFA with $L(M)\subseteq \Sigma^*$. Then,
  $L(M)\in\st{1/2}\cup\{\Sigma^*\}$ if and only if~$M$ does not have a
  subgraph in its transition graph as depicted in the left of
  Figure~\ref{fig:forbidden-pattern-half} with $x,w,z\in \Sigma^*$---see~\cite{Ar91}.
\item Let~$M$ be the minimal DFA with $L(M)\subseteq \Sigma^+$. Then,
  $L(M)\in\dd{1/2}$ if and only if~$M$ does not have a subgraph in its
  transition graph as depicted in the right of
  Figure~\ref{fig:forbidden-pattern-half} with $v,w,z\in
  \Sigma^+$---see~\cite{PiWe97}.
\end{enumerate}

\paragraph{\bf Partially Ordered Automata Variants.}
Nondeterministic finite automata (NFAs) are defined with several
initial states.  A NFA with state set~$Q$, input alphabet~$\Sigma$, initial
states~$I$, and transition function~$\delta$ is a DFA, if $|I|=1$ and
for every $q\in Q$ and letter~$a\in \Sigma$, $|\delta(q,a)|=1$.\todo[color=gray!27]{PW: Can this NFA definition go now? MH: We need the definition of partially ordered automata.
EA: We need to agree if we have a set of initial state or just one initial state.}

Next we define the important property of being partially ordered. For
an automaton~$M$ a state~$q$ is reachable from a state~$p$, written
$p\leq q$, if there is a word $w\in \Sigma^*$ such that
$q\in\delta(p,w)$. An automaton is partially ordered (we use the
prefix po to denote this property), if $\leq $ is a partial
order. Partially ordered DFAs were introduced in~\cite{Si72,BrFi80}
and poNFAs in~\cite{STV01}. Partially ordered automata are sometimes
also called acyclic automata.
%
Another interesting property is confluence, that means that for all
states~$q$ and letters~$a$ and~$b$, if there are transitions
$q_a\in\delta(q,a)$ and $q_b\in\delta(q,b)$, then there is a word
$w\in\{a,b\}^*$ that leads the automaton from both~$q_a$ and~$q_b$
to the same state~\cite{Si74}\todo{EA: Does it need to be the same word $w$?}.

%An automaton~$M$ is a chain reset if and only if~$\leq$ is a total order.

\begin{enumerate}
\item {\bf Deterministic Automata Characterizations.}  A language~$L$
  has a syntactic monoid that is $\mathcal R$-trivial ($\mathcal
  L$-trivial, \resp) if and only if the minimal DFA (that moves the
  head from right to left, \resp) is partially ordered~\cite{BrFi80}.

  When considering confluent poDFAs we find the following situation. A
  language is piecewise testable (i.e., belongs to the
class $\sts{1/2}$) if and only if the minimal DFA
  accepting the language is confluent and partially
  ordered~\cite{KlPo13}. This is equivalent to the so called UMS
  property, which will be discussed in detail for the nondeterminstic
  automata characterizations.

\item {\bf Nondeterministic Automata Characterizations.}  For partial
  NFAs the landscape is more involved. In~\cite{STV01} it was shown
  that poNFAs (with multiple initial states) characterize the
  class~$\sts{3/2}$.

{\tt Markus (I had no time to finish this part in time; will work on that later):

The \emph{unique maximal state property} (UMS) is defined as follows~\cite{Tr01}: An NFA~$M$ on the state set~$Q$ and alphabet~$A$ induces a directed graph $G(M)$ with vertices~$Q$ and where $(p,q)$ is an edge if $q\in\delta(p,a)$, for some~$a$ in~$A$. For $A_1\subseteq A$, we define the graph$G(M,A_0)$ with the set of vertices~$Q$ considered ony those transitions that correspond to letters in~$A_0$. For a state~$p$ let $A(p)=\{\,a\in A\mid p\in\delta(p,a)\,\}$. This is the set of all letters where~$M$ has a self-loop on state~$p$. Let~$M$ be a poNFA. If for every state~$p$ in~$A$, state~$p$ is the unique maximal state of the connected component of $G(M,A(p))$ containing~$p$, then~$M$ has the unique maximal state property.

ptNFA if it is partially ordered, complete, and satisfies the UMS property.

confluence and UMS for NFAs do not coincide. 

A regular language is piecewise testable if and only if it is recognized by a ptNFA~\cite{MaTh15}.

restricted partially ordered NFA is a poNFA such that for every state~$q$ and letter~$a$, if $q\in\delta(q,a)$, then $\delta(q,a)=\{q\}$. 

An $\mathcal R$-expression is a finite union of regular expression of the form $a_)^*a_1A_1^*\cdots a_mA_m^*$, where $m\geq 0$, $a_1,a_2,\ldots,a_m\in A$,\ $A_i\subseteq A$, for $0\leq i\leq m$, and $a_i\not\in A_{i-1}$, for $1\leq i\leq m$. Then let~$L$ be a language described by an $\mathcal R$-expression. The reduced automaton accepting~$L$ is partially ordered~\cite{MeTh69,Fi79}.

\cite{KTM17}: rpoNFAs characterize the class of $\mathcal R$-trivial languages

There is a finer classification of rpoNFAs with single initial state in~\cite{KTM17}

Every rpoNFA language is DRE definable~\cite{KMT17}, that is can be
described by a regular expression where the position automaton is
deterministic~\cite{BrWo98}. Moreover, every language of a minimal
poDFA is DRE-definable~\cite{KMT17}.
}


\end{enumerate}

\burp{to be continued...}

\paragraph{\bf ${\mathcal R}$-, $\mathcal L$-, and $\mathcal J$-trivial Languages.}

\burp{to be continued...}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "sample.tex"
%%% End: 


==> HierarchiesOld.tex <==

\section{\INE\ the Tractable Cases---Inside Logspace} %:  Level~ $0$ and~ $1/2$ of the Straubing-Th{\'e}rien Hierarchy.}
\label{section:INELogspace}

%\todo[inline]{MO: The main insight of this section is Lemma 1 + the first part of Theorem 3. In other words, the 
%clever part is the containment in $\NL$ and in $\L$. The hardness part is more standard. So I would suggest that 
%we split the presentation in two statements: The easy one, showing hardness, and the insightful one, showing containment. 
%The proof of the easy one goes to the appendix. The proof of the insightful one stays.}

A language of~$\Sigma^*$ belongs to level~$0$ of the
Straubing-Th{\'e}rien hierarchy if and only if it is empty
or~$\Sigma^*$. The \INE\ problem for language from this language
family is not entirely trivial, because we have to check for
emptiness. Since by our problem definition the property of a language
being a member of level~$0$ is a promise, we can do the emptiness
check within $\AC^0$, since we only have to verify
whether the empty word belongs to the language~$L$ specified by the
automaton. In case $\varepsilon\in L$, then $L=\Sigma^*$; otherwise
$L=\emptyset$. Since in the definition of finite state devices we do
not allow for $\varepsilon$-transitions, we thus, only have to check
whether the initial state is also an accepting one.  Therefore, we
obtain:

\begin{theorem}\label{thm:STH-0-AC0}
  The \INE\ problem for DFAs or NFAs accepting languages from~$\st{0}$
belongs to $\AC^0$. 
%\todo{MO: I think the best is to state the theorem using logspace uniform $\AC_0$}
\end{theorem}

For the languages of level~$\frac12$ of the Straubing-Th{\'e}rien hierarchy,
we find the following completeness result.

\begin{theorem}\label{thm:NL-completeness}
  The \INE\ problem for NFAs with common unary, fixed, or arbitrary
  size input alphabet accepting languages from~$\st{1/2}$ is
  \NL-complete. If the input instance contains only DFAs, the problem
  becomes \L-complete (under weak reductions\footnote{Some form of
    $\AC^0$ reducibility can be employed.}).
\end{theorem}

Hardness is shown by standard contructions that reduce from variants
of graph accessibility problems~\cite{HIM78,Su75b}.

\begin{lemma}\label{lem:STH-1/2-hardness}
  The \INE\ problem for NFAs with common unary, fixed, or arbitrary
  size input alphabet accepting languages from~$\st{1/2}$ is
  \NL-hard. If the input instance contains only DFAs, the problem
  becomes \L-hard under weak reductions.
\end{lemma}
\begin{toappendix}
\begin{proof}[Proof of Lemma~\ref{lem:STH-1/2-hardness}]
  The \NL-complete graph accessibility problem 2-GAP~\cite{Su75b} is
  defined as follows: given a directed graph $G=(V,E)$ with outdegree
  (at most) two and two vertices~$s$ and~$t$. Is there a path
  linking~$s$ and~$t$ in~$G$?  The problem remains \NL-complete if the
  outdegree of every vertex of~$G$ is exactly two and if the graph is
  ordered, that is, if $(i,j)\in E$, then $i<j$ must be satisfied. The
  complexity of the reachability problem drops to \L-completeness, if
  one considers the restriction that the outdegree is at one. In this
  case the problem is referred to as 1-GAP~\cite{HIM78}.

  First we consider the \INE\ problem for
  NFAs. The \NL-hardness is seen as follows: let $G=(V,E)$ and
  $s,t\in V$ be an ordered 2-GAP instance. Without loss of generality,
  we assume that $V=\{1,2,\ldots,n\}$, the source vertex $s=1$, and
  the target vertex $t=n$. From~$G$ we construct a unary NFA
  $A=(V,\{a\},\delta,1,n)$, where $\delta(i,a)=\{\,j\mid (i,j)\in
  E\,\}\cup\{i\}$.  The 2-GAP instance has a solution if and only if
  the language accepted by~$A$ is non-empty. Moreover, by construction
  the automaton accepts a language of level~$\frac12$, because (i) the
  NFA without $a$-self-loops is acyclic, since~$G$ is ordered, and thus
  does not contain any large cycles and (ii) all states do have
  self-loops.  This proves the hardness and moverover the
  \NL-completeness.

  Finally, we concentrate on the \L-hardness of the
  \INE\ problem for DFAs. Here we use
  the 1-GAP variant to prove our result. Let $G=(V,E)$ and $s,t\in V$
  be a 1-GAP instance, where we can assume that $V=\{1,2,\ldots,
  n\}$,\ $s=1$, and $t=n$. From~$G$ we construct a unary DFA
  $A=(V,\{a\},\delta,1,n)$ with $\delta(i,a)=j$, for $(i,j)\in E$ and
  $1\leq i<n$, and $\delta(n,a)=n$. By construction the DFA~$A$
  accepts either the empty language or a unary language where all
  words are at least of a certain length. In both cases~$L(A)$ is a
  language from level~$\frac12$ of the Straubing-Th{\'e}rien
  hierarchy. Moreover, it is easy to see that there is a path in~$G$
  linking~$s$ and~$t$ if and only if $L(A)\neq\emptyset$. Hence, this
  proves \L-hardness and moreover \L-completeness for an intersection
  non-emptiness instance of DFAs.
\end{proof}
\end{toappendix}

It remains to show containment in logspace. To this end, we utilize an
alternative characterization of the languages of level~$\frac12$ of
the Straubing-Th{\'e}rien hierarchy as exactly those languages that are shuffle
ideals. A
%language~$L$ is a shuffle ideal if for every word~$w\in L$ and
%The languages of level~$\frac12$ of the Straubing-Th{\'e}rien
%hierarchy are excatly those languages that are shuffle ideals.  A
language~$L$ is a shuffle ideal
if, for every word~$w\in L$ and
$v\in\Sigma^*$, the set $w\shuffle v$ is contained in~$L$, where
\begin{multline*}
w\shuffle v:=\{\,w_0v_0w_1v_1\ldots w_kv_k\mid\mbox{$w=w_0w_1\ldots
  w_k$ and $v=v_0v_1\ldots v_k$}\\
\mbox{with $w_i,u_i\in\Sigma^*$, for $0\leq i\leq k$}\,\}.
\end{multline*}
The operation~$\shuffle$
naturally generalizes to sets. 
%It can be decided in deterministic polynomial time whether
%the language accepted by a DFA is of level~$\frac12$.
%
For the \INE{} problem for languages from
level~$\frac12$, we find the following situation.

\begin{lemma}\label{lem:half-level-intersection-nonemptiness-iff-emptiness}
  Let $m\geq 1$ and languages $L_i\subseteq\Sigma^*$, for $1\leq i\leq
  m$, be shuffle ideal, i.e., they belong to the first half level of
  the Straubing-Th{\'e}rien hierarchy. Then,
  $$\bigcap_{i=1}^m L_i\neq\emptyset\quad\mbox{if and only if}\quad L_1L_2\cdots L_m\neq\emptyset.$$ 
  Note that $L_1L_2\cdots L_m$ is a shuffle ideal, too, and that
  $L_1L_2\cdots L_m\neq \emptyset$ if and only if $L_i\neq\emptyset$ 
  for every~$i$ with $1\leq i\leq m$. Finally, $L_i\neq\emptyset$, for
  $1\leq i\leq m$, if and only if $(a_1a_2\ldots a_k)^\ell\in L_i$, where
  $\Sigma=\{a_1,a_2,\ldots a_k\}$ and the shortest word in~$L_i$ is of
  length~$\ell$.
\end{lemma}

\begin{proof}
  The implication from left to right holds, because if
  $\bigcap_{i=1}^m L_i\neq\emptyset$, then there is a word~$w$ that
  belongs to all~$L_i$, and hence the concatenation $L_1L_2\cdots L_m$
  is nonempty, too. Since this argument has not used the prerequisite
  that the~$L_i$'s belong to the first half level of the
  Straubing-Th{\'e}rien hiearchy, this implication does hold in
  general.

  For the converse implication, recall that a language~$L$ of the first
  half level it is a finite (possibly empty) union of languages of the
  form $\Sigma^*a_1\Sigma^*a_2\cdots a_k\Sigma^*$, where the~$a_i$'s
  are letters. Hence, whenever word~$w$ belongs to~$L$, any word of
  the form $uwv$ with $u,v\in\Sigma^*$ is a member of~$L_i$, too. 
  Now assume that $L_1L_2\cdots L_m\neq\emptyset$, which can be wittnessed
  by words $w_i\in L_i$, for $1\leq i\leq m$. But then the word
  $w_1w_2\ldots w_m$ belongs to every~$L_i$, by setting
  $u=w_1w_2\ldots w_{i-1}$ and $v=w_{i+1}w_{i+2}\ldots w_m$ and using
  the argument above. Therefore, the intersection of all~$L_i$, i.e.,
  the set $\bigcap_{i=1}^m L_i$, is nonempty, because of the word
  $w_1w_2\ldots w_m$. 

  The statement that $L_1L_2\cdots L_m$ is an ideal and that
  $L_1L_2\cdots L_m\neq\emptyset$ if and only if~$L_i\neq\emptyset$,
  for every~$i$ with $1\leq i\leq m$, is obvious.

  For the last statement, assume $\Sigma=\{a_1,a_2\ldots,a_k\}$. The
  implication from right to left is immediate, because if $(a_1a_2\ldots
  a_k)^\ell\in L_i$, for~$\ell$ as specified above, then~$L_i$ is
  non-empty. Conversely, if~$L_i$ is non-empty, then there is a
  shortest word~$w$ of length~$\ell$ that is contained in~$L_i$. But then
  $(a_1a_2\ldots a_k)^\ell$ belongs to $w\shuffle\Sigma^*$, which by
  assumption is a subset of the language~$L_i$, since~$L_i$ is an
  ideal. Therefore, $L_i\neq\emptyset$ implies $(a_1a_2\ldots
  a_k)^\ell\in L_i$, which proves the stated claim.
\end{proof}
Now we are ready to prove containment in logspace.
\begin{lemma}
  The \INE\ problem for NFAs with common unary, fixed, or arbitrary
  size input alphabet accepting languages from~$\st{1/2}$ belongs to
  \NL. If the input instance contains only DFAs, the problem is
  solvable in \L.
\end{lemma}

\begin{proof}
  In order to solve the \INE\ problem  
  for given finite automata $A_1,A_2,\ldots, A_m$ with a common input
  alphabet~$\Sigma$, regardless of whether they are deterministic or
  nondeterministic, it suffices to check non-emptiness for all
  languages~$L(A_i)$, for $1\leq i\leq m$, in sequence, because of
  Lemma~\ref{lem:half-level-intersection-nonemptiness-iff-emptiness}. To
  this end, membership of the words $(a_1a_2\ldots a_k)^{\ell_i}$
  in~$L_i$ has to be verified, where~$\ell_i$ is the length of the
  shortest word in~$L_i$. Obviously, all~$\ell_i$ are linearly bounded
  in the number of states of the appropriate finite automaton that
  accepts~$L_i$. Hence, for an NFA input instance, the verification
  can be done on a nondeterministic logspace-bounded Turing machine,
  guessing the computations in the individual NFAs---we do not have to
  guess the input word to the NFAs here, since it can be chosen to be
  $(a_1a_2\ldots a_k)^{\ell_i}$. Therefore, for a DFAs input instance,
  nondeterminism is not needed, and thus the overall procedure can be
  implemented on a determinstic Turing machine. Thus, the \INE\ problem
  for NFAs belongs to \NL, while it is contained in \L\ for DFAs.
\end{proof}


\section{\INE\ Intractable Cases: \NP-Hardness and -Completeness}
In contrast to the Straubing-Thérien hierarchy, the \INE problem for languages from the dot-depth hierarchy is already \NP-hard in the lowest level $\dd{0}$. As a result, the \INE problem for languages from the Straubing-Thérien hierarchy of level $\st{1}$ and above is also \NP-hard. More precisely, we prove that the \INE problem is \NP-hard, even if only one automaton $A_i$ from the input DFAs accepts a language from $\st{1}$ and all other DFAs $A_j$ with $i \neq j$ accept languages from $\st{1/2}$. 
For the levels  $\dd{0}$,\ $\dd{1/2}$,\ $\st{1}$, or~$\st{3/2}$ we give matching complexity upper bounds if the input automata are DFAs, yielding the first main result of this section proven in Subsection~\ref{sec:NP-hardness} and~\ref{sec:NP-membership}.
\begin{theorem}
	\label{thm:NPCompleteness}
	The \INE problem for DFAs accepting languages from either $\dd{0}$, $\dd{1/2}$, $\st{1}$, or~$\st{3/2}$ is \NP-complete. The same holds for poNFAs instead of~DFAs. The results hold even for a binary alphabet.
\end{theorem}


For the level $\dd{0}$ we obtain a complete picture of the complexity of the \INE problem, independent on structural properties of the input finite automata, i.e., we show that here the problem is \NP-complete for general NFAs. For the levels $\dd{1/2}$,\ $\st{1}$,\ and $\st{3/2}$ we show that the \INE problem is \NP-complete if the input automata are in the class of automata characteristic\todo{PW: Can I use 'characteristic' in this context?
SH: Could be interpreted to mean these models characterize the mentioned class, which is not the case for poDFAs and $\st{1}$ and poNFAs and $\dd{1/2}$. So, I would make the wording more clear, or different, here.} for the corresponding language class, that are poDFAs for $\st{1}$ and poNFAs for $\dd{1/2}$ and $\st{3/2}$.

For the level $\dd{0}$, we obtain a complete picture of the complexity of the \INE problem, independent on structural properties of the input finite automata, i.e., we show that here the problem is \NP-complete for general NFAs. For the levels $\dd{1/2}$,\ $\st{1}$,\ and $\st{3/2}$ we show that the \INE problem is \NP-complete if the input automata are in the class of automata characteristic\todo{PW: Can I use 'characteristic' in this context?} for the corresponding language class, that are poDFAs for $\st{1}$ and poNFAs for $\dd{1/2}$ and $\st{3/2}$.

If the input automata are given as NFAs without any structural property, then the precise complexity of \INE for $\dd{1/2}$,\ $\st{1}$,\ and $\st{3/2}$ is an open problem and narrowed by \NP-hardness and membership in \PSPACE. We present a ``No-Go-Theorem'' by proving that for an NFA $A$ accepting a co-finite language, the smallest poNFA $B$ that is equivalent to $A$ is exponentially larger than $A$ as our second main result of this section proven in Section~\ref{sec:LargePONFA}.

\begin{restatable}{theorem}{RestateThmLargePoNFA}\label{thm:largePONFA}
	For every $n \in \mathbb{N}$, there exists a language $L_n \in \dd{0}$ on a binary alphabet
	such that $L_n$ is recognised by an NFA of size $n(2n+5)$,
	but the minimal poNFA recognising $L_n$ has more than $2^{n-1}$ states.
\end{restatable}



\subsection{\NP-hardness}
\label{sec:NP-hardness}

\todo[inline]{MO: I think that most material of this subsection should be removed and more or less replaced by the sketch in red below.
The issue is that Lemma \ref{lem:NP-hard-FiniteLang} is statement is Theorem 1 of \cite{Rampersad2010detecting} and the proof is the same.
It seems that the best is to prove Theorem \ref{thm:ST-1-NP-hard} directly, by adapting the proof from \cite{Rampersad2010detecting}}
\textcolor{red}{
(SKETCH FOR THIS SECTION)}
\\ 
\textcolor{magenta}{THE MAIN RESULT OF THIS SECTION IS THAT FOR DFAs THE \INE PROBLEM IS ALREADY NP-COMPLETE IF ONLY ONE LANGUAGE IS FROM $\st{1}$ AND ALL OTHER LANGUAGES ARE FROM $\st{1/2}$.}
\begin{lemma}[Theorem 1 of \cite{Rampersad2010detecting}]
The \INE problem for DFAs all accepting finite binary languages is \NP-complete.
\end{lemma}
Since finite languages belong to $\dd{0}$, $\dd{1/2}$, $\st{1}$ and $\st{3/2}$ we have the following corollary. 
\begin{corollary}
\label{NPHardnessBZero}
	The \INE problem is \NP-hard when all input automata are DFAs accepting languages in one of the levels $\dd{0}$, $\dd{1/2}$, $\st{1}$ or $\st{3/2}$. 
\end{corollary}
\begin{remark}
	Recall, that the dot-depth hierarchy, apart form~$\dd{0}$, coincides with the concatenation hierarchy starting with the language class $\{\emptyset,\{\lambda\},\Sigma^+,\Sigma^*\}$. The \INE problem for DFAs or NFAs accepting only languages from $\{\emptyset,\{\lambda\},\Sigma^+,\Sigma^*\}$ belongs to $\AC^0$, by similar arguments as in the proof of Theorem~\ref{thm:STH-0-AC0}.
\end{remark}
We have shown in Section \ref{section:INELogspace} that \INE for NFAs, all accepting languages in $\st{1/2}$, belongs to $\NL$. The main theorem of this section states 
that already in the DFA case, if we allow only one of the DFAs in the list to accept a language from $\st{1}$, then the problem becomes \NP-hard. The statement also holds if the common alphabet is binary. 
\begin{theorem}\label{thm:ST-1-NP-hard}
	The \INE problem \textcolor{red}{for DFAs} is \NP-hard even if only one DFA accepts a language from $\st{1}$ and all other DFAs accept languages
	from~$\st{1/2}$ and the alphabet is binary.
\end{theorem}
\begin{proofsketch}
	The proof is by a reduction from the \textsc{Vertex Cover} problem. Let $G = (V, E)$ be an undirected graph with $n$ nodes and $m$ edges and let $k\in \mathbb{N}$. 
	Each word $w$ accepted by all $m+1$ automata will be of size exactly $n$ and will represent an encoding of a vertex cover of size at most~$k$. Therefore, $w$ has a $1$ at position $j$ if and only if the vertex $v_j$ is in the vertex cover. We define for each edge $e_i \in E$ with $e_i = \{v_{i_2}, v_{i_2}\}$ an automaton~$A_{e_i}$ that checks that $w[i_1] = 1$ or $w[i_2] = 1$. Here, $w[i]$ refers to the $i$th letter in the word~$w$. We allow $A_{e_i}$ to read before and after the positions $i_1$ and $i_2$ arbitrary strings, but ensure that $A_{e_i}$ accepts only words of size at least $n$. Therefore, $A_{e_i}$ accepts the language $\Sigma^{\geq i_1 - 1}\cdot1\cdot\Sigma^{\geq n-i_1} \cup
	\Sigma^{\geq i_2 - 1}\cdot1\cdot\Sigma^{\geq n-i_2}
	\cup
	\Sigma^{\geq 2n-1}$ of level $\st{1/2}$. The most difficult part is to construct $A_{e_i}$ as a \emph{deterministic} automaton of size $\mathcal{O}(n^2)$. 
	The only language from level $\st{1}$ is the finite language of all word of size \emph{exactly} $n$ that contain at most $k$ appearances of the letter $1$.
%	The proof is an adaption of the reduction from \textsc{3-CNF-SAT} in the proof of~\cite[Theorem~1]{Rampersad2010detecting}. There, for a 3-CNF formula $\varphi$ over $n$ variables and $m$ clauses, for each clause $c$, a DFA $A_c$ accepting a finite language of words of length $n$ is constructed. Hereby, a binary word of length $n$ encodes a variable assignment of $n$ variables. Each automaton~$A_c$ then accepts all encoded assignments that satisfy the clause $c$. We now adapt this construction by adding self-loops to all states of the automata~$A_c$ such that their language is contained in $\st{1/2}$ (and $A_c$ becomes non-deterministic). Note that now each $A_c$ accepts an infinite language where all words are of size at least $n$. To enforce that none of the intermediate self-loops can actually be taken, we add a DFA $A_{\leq n}$ to the sequence of automata that accepts all binary words of size at most $n$. As this is the complement of the $\st{1/2}$ language $\{0, 1\}^{\geq n}$, $L(A_{\leq n})$ is the only language from $\st{1}$ in the intersection.
\end{proofsketch}
\todo[inline]{Begin toappendix}


%This subsection is denoted to the \NP-hardness part of the proof of Theorem~\ref{thm:NPCompleteness}.
%For the NP-hardness proof for the level $\dd{0}$ of the dop-depth hierarchy, we adapt a construction, independently given by Eppstein~\cite{DBLP:journals/siamcomp/Eppstein90} and Rystsov~\cite{DBLP:journals/ipl/Rystsov83} for the problem of finding a shortest synchronizing word for a given DFA. Therefore, we make the implicit conjunction of end states of all parallel runs in a synchronizing automaton explicit by splitting the automaton
%%	 in the construction from \cite{} 
%into several automata all accepting finite languages.
%All of our constructed automata will be partially ordered DFAs. The named construction has been adapted to synchronization problems of partially ordered automata in~\cite[Theorem~4]{DBLP:journals/tcs/Ryzhikov19a} and from there adapted to show \NP-completeness of the  \textsc{Intersection Non-emptiness Problem} for DFAs
%with the property of being partially ordered~\cite[Proposition~9]{DBLP:journals/tcs/Ryzhikov19a}. Recall that partially ordered DFAs characterize a class of languages that is strictly between $\st{1}$ and~$\st{3/2}$.
%Here, we improve the construction to show that the \INE problem is already \NP-hard if all input DFAs accept finite languages. Recall, that all finite languages are contained in $\dd{0}$.
%
%
%
%In order to prove Theorem~\ref{thm:ST-1-NP-hard}, we give a reduction from the satisfiability problem for formulas in conjunctive normal form where every clause contains exactly three literals (in 3-CNF for short):
%\begin{definition}[\textsc{3-CNF-SAT}]\  \\
%	Input: Boolean formula $\varphi$ given as a set of clauses $C=\{c_1, c_2, \dots, c_m\}$ over a set of variables $V=\{x_1, x_2, \dots, x_n\}$ such that $|c_i|\leq3$ for $i\leq m$.\\
%	Output: Is there a variable assignment $\beta \colon V \to \{0,1\}$ such that $\varphi$ evaluates to true under $\beta$?
%\end{definition}
In order to prove \autoref{thm:ST-1-NP-hard} we give a reduction from the \textsc{Vertex Cover} problem.
\begin{definition}[\textsc{Vertex Cover}]\  \\
	Input: Undirected graph $G=(V, E)$ with vertex set $V$ and edge set $E \subseteq V \times V$ and integer $k$. \\
	Output: Is there a subset $S \subseteq V$ with $|S| \leq k$ and for all $e \in E$, $S \cap e \neq \emptyset$? \\
	If yes, we call $S$ a \emph{vertex cover} of $G$ of size at most $k$. 
\end{definition} 

%\begin{theorem}\label{thm:DD-1/2-NP-hard}
%	The intersection non-emptiness problem for DFAs all accepting languages
%	from~$\dd{1/2}$ %or $\ddp{1/2}$ 
%is \NP-hard.
%\end{theorem}
%\begin{lemma}\label{lem:NP-hard-FiniteLang}
%	The \INE problem for DFAs all accepting finite binary languages is \NP-hard.
%\end{lemma}
\begin{proof}[Proof of Theorem~\ref{thm:ST-1-NP-hard}]
    Let $k\in \mathbb{N}$ and let $G = (V, E)$ be an undirected graph with vertex set $V = \{v_0, v_2, \dots, v_{n-1}\}$ and edge set $E= \{e_0, e_2, \dots, e_{m-1}\}$.
    From $(G, k)$ we construct $m+1$ DFAs over the common alphabet $\Sigma = \{0, 1\}$. The input word for these automata will encode which vertices are in the vertex cover. Therefore, we assume a linear order on $V$ indicated by the indices of the vertices. More precisely, a word accepted by all automata will have a $1$ at position $j$ if and only if the vertex $v_j$ will be contained in the vertex cover $S$. For a word $w=w_1w_2\dots w_l$ with $w_j \in \Sigma$ for $1\leq j \leq l$ we denote $w[j]=w_j$. We may call a word $w$ of length $n$ a \emph{vertex cover} and say that the vertex cover covers an edge $e = \{v_{j_1}, v_{j_2}\}$ if $w[j_1] = 1$ or $w[j_2] = 1$.
	
	For every edge $e_i\in E$ with $e_i = \{v_{i_1}, v_{i_2}\}$, $i_1 < i_2$, we construct a DFA $A_{e_i}$ consisting of $i_1 - i_2 +2$ chains, where one is of length $2n-1$, one of length $n-(i_2+1)$, and all others are of length $n-(i_1+1)$. The DFA is defined as $A_{e_i} = (Q, \Sigma, \delta, q^0, F)$ with state set 
	$Q = \{\,q^j \mid 0 \leq j \leq 2n-1\,\} \cup \{\,{q'}_\ell^j \mid i_1+1 \leq j \leq n, 1 \leq \ell \leq i_1 -i_2\,\} \cup \{\,{q''}^j \mid i_2+1 \leq j \leq n\,\}$
    and final states $F = \{q^{2n-1}, {q''}^n\} \cup \{{q'}_\ell^n \mid 1 \leq \ell \leq i_2-i_1 \}$.
    We first focus on the states $\{\,q^j \mid 0 \leq j \leq 2n-1\,\}$. The idea is that there, the first $n$ states correspond to the sequence of vertices and a read $1$ at position $j$ for which $v_j \in e_i$ will cause the automaton to switch to the chain consisting of states ${q'}_1^j$ or ${q''}^j$ depending on whether $v_j = v_{i_1}$ or $v_j=v_{i_2}$. There, only one state is accepting namely the state that we reach after reading a vertex assignment of length exactly $n$ that satisfies the edge $e_i$.
	To be more formal, we define
    $\delta(q^{i_1}, 1) = {q'}_1^{i_1+1}$ and $\delta(q^{i_2}, 1) = {q''}^{i_2+1}$.
%	 for $j \leq n-1$, we define  $\delta_i(q_i^j, 1) = q_i^{j+n}$ if $v_{j+1} \in e_i$. 
    At the moment, think of the remaining undefined transitions as leading to the next state in the sequence.\todo{EA: I think formally defining the transition in the sequence at the beginning may help to understand what a sequence is.}

	
%	For every clause $c_i\in C$, we construct a DFA $A_{c_i}$ consisting of a two phased chain of length $2n$ as $A_{c_i} = (\{\,q_i^j \mid 0 \leq j \leq 2n-1\,\}, \Sigma, \delta_i, q_i^0, \{q_i^{2n-1}\})$. The first $n$ states correspond to the sequence of variables and a read variable assignment that satisfies $c_i$ will cause the automaton to bypass the rest of the states in this part and jump to the corresponding part of the second half of the chain. There, only one state is accepting namely the state that we reach after reading an assignment of exactly $n$ variables which satisfies the clause $c_i$. 
%	To be more formal, for $j \leq n-1$, we define $\delta_i(q_i^j, 0) = q_i^{j+n}$ if $\neg x_{j+1} \in c_i$, and  $\delta_i(q_i^j, 1) = q_i^{j+n}$ if $x_{j+1} \in c_i$. At the moment, think of the remaining undefined transitions as leading leading to the next state in the sequence.
	
	
%	, and  $\delta_i(q_i^j, \sigma) = q_i^{j+1}$ otherwise, for $\sigma\in \Sigma$ that does not fall under the two previous cases. We further define $\delta_i(q_i^j, \sigma) = q_i^{j+1}$ for $n\leq j < 2n-1$ and $\sigma\in \Sigma$.


    So far, $A_{e_i}$ accepts a finite language where all accepted words are of size at least $n$. In order to integrate the accepted language of $A_{e_i}$ into $\st{1/2}$ we need to allow $A_{e_i}$ to read an arbitrary word between each letter causing a state transition, i.e., if $A_{e_i}$ accepts the word $w = w_1 w_2 \dots w_l$, then we need to add the language $\Sigma^* w_1 \Sigma^* w_2 \dots w_l \Sigma^*$ to $L(A_{e_i})$. 
	In order to do this modification while preserving the determinism of $A_{e_i}$, we make the following observations.
%	 where for $1\leq j \leq 2$, $v_{i_j}$ is a literal of the variable $x_{i_j}$ and let $\sigma_{i_j}$ be $1$ if $\ell_{i_j}$ is a positive literal and $0$, otherwise. 
%	Then, 
	\[L(A_{e_i}) = 
	\Sigma^{i_1 - 1}\cdot1\cdot\Sigma^{n-i_1} \cup
	\Sigma^{i_2 - 1}\cdot1\cdot\Sigma^{n-i_2}
	\cup
	\Sigma^{2n-1}.
	\]
	Introducing a self-loop labeled with $\Sigma$ would change the language $L(A_{e_i})$ to the following language of level $\st{1/2}$.
	\begin{align*}
		L_{e_i} &= 
		\Sigma^{i_1 - 1}\Sigma^*\cdot1\cdot\Sigma^{n-i_1}\Sigma^* \cup
		\Sigma^{i_2 - 1}\Sigma^*\cdot1\cdot\Sigma^{n-i_2}\Sigma^*
		\cup
		\Sigma^{2n-1}\Sigma^*\\
		&=
		\Sigma^{\geq i_1 - 1}\cdot1\cdot\Sigma^{\geq n-i_1} \cup
		\Sigma^{\geq i_2 - 1}\cdot1\cdot\Sigma^{\geq n-i_2}
		\cup
		\Sigma^{\geq 2n-1}\\
		&=
		\Sigma^{\geq 2n-1}\, \cup \,  
		\bigcup_{\alpha \leq n - 2 } \Sigma^{i_1-1}\, 0^\alpha\, 1\, \Sigma^{n-i_1} \Sigma^*
		\cup
		\bigcup_{\alpha \leq n - 2 } \Sigma^{i_2-1}\, 0^\alpha\, 1\, \Sigma^{n-i_2} \Sigma^*.
    \end{align*}
%	Denote for $\sigma_{i_j}$ with $\overline{\sigma}_{i_j} = \Sigma\setminus\{\sigma_{i_j}\}$ the negation of $\sigma_{i_j}$ interpreted as a Boolean value.
%	Note that for each $i_j$, 
%	\[\Sigma^{\geq 2n-1}\, \cup \, \Sigma^{\geq i_j -1}\sigma_{i_j} \Sigma^{\geq n-i_j} = \Sigma^{\geq 2n-1}\, \cup \,  \bigcup_{\alpha \leq n+ i_j -3 } \Sigma^{i_j-1}\, \overline{\sigma}_{i_j} {}^\alpha\, \sigma_{i_j}\, \Sigma^{n-i_j} \Sigma^*.\]
%	This language can be accepted by the DFA $A_{i_j} = (\{\,q_i^j \mid 0 \leq j \leq 2n-1\,\}, \Sigma, \delta_i, q_i^0, \{q_i^{2n-1}\})$ where $\delta$ is defined according to the state graph of $A_{i_j}$ depicted in Figure~\ref{fig:st-1-2-lineDFA}.
	We now define the missing transitions for $A_{e_i}$ such that $A_{e_i}$ stays deterministic but accepts the language above, i.e., that $L(A_{e_i}) = L_{e_i}$.
	The state graph of $A_{e_i}$ is depicted in Figure~\ref{fig:st-1-2-lineDFA}.
	\begin{figure}
		\centering
		\begin{tikzpicture}[scale=0.4,inner sep=1pt,->,>=stealth',shorten >= 1pt,auto,node distance = 1.3cm,semithick, initial text =,state/.style={circle, draw,minimum size=0.8cm, initial text = }] 
				\node[state, initial] (0) {0};
				\node[state, right of=0, node distance = 1.6cm] (1) {\scalebox{0.6}{$i_1$}};
				\node[state, right of=1] (2) {\scalebox{0.6}{$i_1$+$1$}};
				\node[state, right of=2, node distance = 1.6cm] (3) {\scalebox{0.6}{$i_2$-1}};
				\node[state, right of=3] (4) {\scalebox{0.6}{$i_2$}};			
				\node[state, right of=4] (5) {\scalebox{0.6}{$i_2$+$1$}};
				\node[state, right of=5, node distance = 1.6cm] (6) {\scalebox{0.6}{$n$+$i_2$}};
				\node[state, right of=6] (62) {\scalebox{0.6}{$n$+$i_2$+$1$}};
				\node[state, accepting, right of=62, node distance = 1.6cm] (6') {\scalebox{0.6}{$2n$-$1$}};
%				\node[below of=4] (ghost) {};
				
				
				
				
				
				\node[state, below of=1, node distance = 1.6cm] (7) {\scalebox{0.6}{$i_1$+$1$}};
				\node[state, left of=7] (8) {\scalebox{0.6}{$i_1$+$2$}};
				\node[state, accepting, left of=8, node distance = 1.6cm] (8') {\scalebox{0.6}{$n$}};
				
				\node[state, below of=7, node distance=1.5cm] (c7) {\scalebox{0.6}{$i_2$-$1$}};
				\node[state, left of=c7] (c8) {\scalebox{0.6}{$i_2$}};
				\node[state, accepting, left of=c8, node distance = 1.6cm] (c8') {\scalebox{0.6}{$n$}};
				\node[state, right of=c7] (c6) {\scalebox{0.6}{$i_1$+$2$}};
				\node[state, right of=c6] (c5) {\scalebox{0.6}{$i_1$+$1$}};
			
				\node[below of=c7, node distance= 0.7cm] (ghost) {};
				\node[left of=ghost] (dots) {$\vdots$};
				
				\node[state, below of=ghost, node distance=1cm] (cc7) {\scalebox{0.6}{$i_2$-$\ell$+$1$}};
				\node[state, left of=cc7] (cc8) {\scalebox{0.6}{$i_2$-$\ell$+2}};
				\node[state, accepting, left of=cc8, node distance = 1.6cm] (cc8') {\scalebox{0.6}{$n$}};
				\node[state, right of=cc7] (cc6) {\scalebox{0.6}{$i_1$+$2$}};
				\node[state, right of=cc6] (cc5) {\scalebox{0.6}{$i_1$+$1$}};
				
				\node[state, below of=4, node distance = 1.6cm] (9) {\scalebox{0.6}{$i_2$+$1$}};
				\node[state, right of=9] (10) {\scalebox{0.6}{$i_2$+$2$}};
				\node[state, accepting, right of=10, node distance = 1.6cm] (11) {\scalebox{0.6}{$n$}};
				
				
				\path
				(0) edge[dotted] node[pos=0.4] {$\Sigma$} (1)
				(1) edge node[pos=0.4] {$0$} (2)
				(1) edge node[pos=0.2] {$1$} (7)
				(2) edge[dotted] node[pos=0.4] {$0$} (3)
				(2) edge[bend left=10] node[pos=0.2] {$1$} (c5)
				(3) edge node[pos=0.4] {$0$} (4)
				(3) edge[bend left=20] node[pos=0.2] {$1$} (cc5)
				(4) edge node[pos=0.4] {$0$} (5)
				(4) edge node[pos=0.2] {$1$} (9)
				(5) edge[dotted] node[pos=0.4] {$0$} (6)
				(5) edge[bend right=10] node[pos=0.2] {$1$} (9)
				(6) edge[bend right=10] node[pos=0.2] {$1$} (9)
				(6) edge[pos=0.4] node {$0$} (62)
				(62) edge[dotted, pos=0.4] node {$\Sigma$} (6')
				(6') edge[loop below] node {$\Sigma$} (6')
				%
				%
				%
				(7) edge node[pos=0.4, above] {$\Sigma$} (8)
				(8) edge[dotted] node[pos=0.4, above] {$\Sigma$} (8')
				(8') edge[loop above] node[left, pos=0.1] {$\Sigma$} (8')
				%
				(c7) edge node[pos=0.4, above] {$0$} (c8)
				(c7) edge[bend right=60] node[pos=0.05, below] {$1$} (9)
				(c8) edge[dotted] node[pos=0.4, above] {$0$} (c8')
				(c8) edge[bend right=50] node[pos=0.05, below] {$1$} (10)
				(c8') edge[loop above] node[left, pos=0.1] {$\Sigma$} (c8')
				(c5) edge node[pos=0.4, above] {$\Sigma$} (c6)
				(c6) edge node[pos=0.4, above] {$\Sigma$} (c7)
				%
				(cc7) edge node[pos=0.4, above] {$0$} (cc8)
				(cc7) edge[bend right=100] node[pos=0.05, below] {$1$} (9)
				(cc8) edge[dotted] node[pos=0.4, above] {$0$} (cc8')
				(cc8) edge[bend right=80] node[pos=0.05, below] {$1$} (10)
				(cc8') edge[loop above, above] node[left, pos=0.1] {$\Sigma$} (cc8')
				(cc5) edge node[pos=0.4, above] {$\Sigma$} (cc6)
				(cc6) edge node[pos=0.4, above] {$\Sigma$} (cc7)
				%
				%
				%
				(9) edge node[pos=0.4] {$\Sigma$} (10)
				(10) edge[dotted] node[above, pos=0.4] {$\Sigma$} (11)
				(11) edge[loop below] node {$\Sigma$} (11);
				
		\end{tikzpicture}
        \vspace{-1cm}
		\caption{DFA $A_{e_i}$ accepting the language $\Sigma^{\geq i_1 - 1}\cdot1\cdot\Sigma^{\geq n-i_1} \cup
			\Sigma^{\geq i_2 - 1}\cdot1\cdot\Sigma^{\geq n-i_2}
			\cup
			\Sigma^{\geq 2n-1}$. A dotted transition between some state $j$ and $j'$ represents a chain containing $j'-j$ copies of the state $j$ adapting the behavior of state $j$. \textcolor{red}{Is this clear?}}
		\label{fig:st-1-2-lineDFA}
	\end{figure}
    \todo{EA: You can use \\useasboundingbox to fix the bounding box before drawing the edges}
	
%	We now describe, how we combine the DFAs $A_{i_j}$ depicted in Figure~\ref{fig:st-1-2-lineDFA} for $1 \leq j \leq 3$, into one DFA $A_{c_i}$. Recall that $\bigcup_{1 \leq j \leq 3} L(A_{i_j}) = L(A_{c_i})$.
%	Assume w.l.o.g.~$i_1 < i_2 < i_3$. We start with the automaton $A_{i_1}$. If $\sigma_{i_2} = \overline{\sigma}_{i_1}$, then,
	
%	
%	This would 
%	 i.e., we add the transitions $\delta(q_i^j, \sigma) = q_i^j$ for all $\sigma \in \Sigma$, $0 \leq j \leq 2n-1$.
	 
    Recall, that we already defined $\delta(q^{i_1}, 1) = {q'}_1^{i_1+1}$ and $\delta(q^{i_2}, 1) = {q''}^{i_2+1}$. We now need to allow to ``miss'' the state $q^{i_1}$ but still be able to take the shortcut into the shorter chain in case we read some more than $i_1-1$ letters in the first $\Sigma^{\geq i_1-1}$ part of the language $\Sigma^{i_1 - 1}\Sigma^*\cdot1\cdot\Sigma^{n-i_1}\Sigma^*$ in $L_{e_i}$. If we took the shortcut to some chain corresponding to $i_1$, we must be able to remember the progress we made on the first chain between the state $q^{i_1}$ and $q^{i_2}$ since we might have ``guessed wrong'' by jumping into the chain associated with $i_1$ with a $1$ but instead are in the part $\Sigma^{\geq i_2-1}$ of $L_{e_i}$. Therefore, we have not only one chain associated with $i_1$ but $i_2 - i_1$ many instances of the chain ${q'}_1^j$, $i_1 +1 \leq j \leq n$.
	Hence, for $i_1 < j < i_2$ we define $\delta(q^j, 1) = {q'}_\ell^{i_1+1}$ with $\ell = j-i_1 +1$. 
    If we already read at least $i_2-1$ letters, than we can surely take the second shortcut into the shorter chain, associated with~$i_2$, if we read a $1$ and the distance to the accepting state of the long chain is still longer than the length of the short chain associated with~$i_2$. In that case, i.e., when we are in a state $q^{j}$ for $i_2 \leq j \leq n+i_2$\todo{EA: changed $n+i_2+1$ to $n+i_2-1$\\
    PW: changed $n+i_2-1$ to $n+i_2$ to be consistent with the picture, indeed both variants work.}, we no longer need to remember our progress in the long chain and can map all states to ${q''}^{i_2+1}$. More formally, we define $\delta(q^j, 1) = {q''}^{i_2+1}$ for $i_2 \leq j \leq n+i_2$\todo{EA: added for $i_2 \leq j \leq n+i_2-1$ PW:changed to $n+i_2$}. If we passed the state $q^{n+i_2}$\todo{EA: changed $n+i_2+1$ to $n+i_2-1$ PW: changed $n+i_2-1$ to $n+i_2$}, then it is shorter to reach the accepting trap state on the long chain than to go through some of the shorter chains. This observation allows us to define $\delta$ for the long chain completely by setting $\delta(q^j, \sigma) = q^{j +1}$ for $0 \leq j \leq i_1-1$ and both $\sigma \in \Sigma$; $\delta(q^j, 0) = q^{j+1}$ for $i_1 \leq j \leq n+i_2$\todo{EA: changed $n+i_2$ to $n+i_2-1$ PW: changed to $n+i_2$}; $\delta(q^j, \sigma) = q^{j +1}$ for $n+i_2 +1 \leq j \leq 2n-2$\todo{EA: changed $n+i_2+1$ to $n+i_2$ PW: changed back}; and $\delta(q^{2n-1}, \sigma) = q^{2n-1}$ for both $\sigma \in \Sigma$.
    As discussed before, in the case we read a first $1$ at position $j$ after at least $i_1$ and at most $i_2$ symbols and then read a second $1$ after at least $i_2$ and at most $n$ symbols in total, we need to jump from the chain associated with $i_1$ to the shorter chain associated with $i_2$ while carrying over the progress we made in the chain of $i_1$. Hence, we define for $1 < \ell \leq i_2-i_1$, $\delta({q'}_\ell^j, 1) = {q''}^{i_2+\ell}$\todo{EA: changed $i_2+\ell$ to $i_2+1$\\ PW: no, this is exactly the progress we saved in the chain index. I changed it back} for $i_2 - \ell +1 \leq j \leq n-\ell$ and $\delta({q'}_\ell^j, 1) = {q''}^{n}$ for $n-\ell+1 \leq j \leq n-1$\todo{EA: changed $i_2 - \ell +1$ to $i_2 - \ell$ and $n - \ell$ to $i_2 - 1$ and removed "and $\delta({q'}_\ell^j, 1) = {q''}^{n}$ for $n-\ell \leq j \leq n-1$"\\PW: no this is the progress that needs to be stored, see figure, I chanted it back}. For all other undefined transitions $\delta({q'}_\ell^j, \sigma)$ with $i_1+1 \leq j \leq n-1$ we define   $\delta({q'}_\ell^j, \sigma) = \delta({q'}_\ell^{j+1})$. Finally, we define $\delta({q'}_\ell^{n}, \sigma) = {q'}_\ell^n$ for both $\sigma \in \Sigma$.
	The only transitions which remain to be defined are in the chain associated with $i_2$. Here, we define $\delta({q''}^{j}, \sigma) = {q''}^{j+1}$ for $i_2+1 \leq j \leq n-1$ and $\delta({q''}^n, \sigma) = {q''}^{n}$ for both $\sigma\in \Sigma$.
	
	Next, we define a DFA $A_{= n, \leq k}$ which accepts the finite language of all binary words of length $n$ which contain at most $k$ appearances of the letter $1$. But first, observe that if we add $A_{= n, \leq k}$ to the sequence of DFAs in the \INE instance, then the only words accepted by each DFA $A_{e_i}$ that may be accepted by all automata are of length \emph{exactly} $n$ and hence are accepted in $A_{e_i}$ either by the state ${q'}_1^n$ or ${q''}^n$. Especially, none of the states ${q'}_\ell^j$ for $\ell > 1$, $i_1+1 \leq j \leq n$ as well as none of the states $q^j$ for $j \geq i_2+1$ can be reached while reading those words.
    By the construction of $A_{e_i}$ words of length exactly~$n$ which are accepted from $A_{e_i}$ have a $1$ at position $i_1$ or at position $i_2$.
	
    We now proceed with defining the automaton $A_{= n, \leq k} = (\{q_i^j \mid 0 \leq i \leq n+1, 0 \leq j \leq k+1\}, \Sigma, \delta, q_0^0, \{q_n^j \mid j \leq k\})$. The state graph of $A_{= n, \leq k}$ is a grid graph, where each letter increases the $x$ dimension represented by the sub-script $i$ up to the value $n+1$, and each letter that is a $1$ increases the $y$ dimension represented by the super-script $j$ up to the value $k+1$. More formally, we define $\delta(q_i^j, 0) = q_{i+1}^j$, and $\delta(q_i^j, 1) = q_{i+1}^{j+1}$ for $0 \leq i \leq n$, $0 \leq j \leq k$; and $\delta(q_{i}^j, \sigma) = q_i^j$ for $i = n+1$ or $j = k+1$. The size of $A_{= n, \leq k}$ is bounded by $\mathcal{O}(nk)$. For readability, we defined $A_{n, \leq k}$ as a non-minimal DFA. As $L(A_{=n, \leq k})$ is finite, it is of level $\dd{0} \subseteq \st{1}$.
	
	Note that each automata $A_{e_i}$ is of size $\mathcal{O}(n^2)$.
	By the arguments discussed in detail above, the set of words accepted by all of the automata $(A_{e_i})_{e_i \in E}$, $A_{= n, \leq k}$ are of size exactly $n$ and encode a vertex cover of size at most $k$ for $G$.
	 %
%	Note that words which correctly encode a complete vertex assignment for $V$ are of size exactly $n$. Hence, in order to forbid $A_{e_i}$ to take any of the introduced self-loops, we add a DFA $A_{\leq n}$ that accepts all words of length at most $n$ to the sequence of automata in the intersection. Note that $L(A_{\leq n})$ is the complement of an $\st{1/2}$ language being defined as the finite union $\bigcup_{\sigma_\ell \in \Sigma, \ell \leq n+1} \Sigma^* \sigma_1 \Sigma^* \sigma_2 \dots \sigma_{n+1} \Sigma^*$. 
%	Hence, $L(A_{\leq n})$ is a language from $\st{1}$.
%	For the sake of completeness we construct $A_{\leq n}$ as $A_{\leq n} = (\{q_0, q_1, \dots, q_{n+1}\}, \Sigma, \delta, q_0, \{q_0, q_1, \dots, q_n\})$ with $\delta(q_\ell, \sigma) = q_{\ell+1}$ for $\sigma\in\Sigma$ and $0 \leq \ell \leq n$; and $\delta(q_{n+1}, \sigma) = q_{n+1}$ for $\sigma \in \Sigma$.
%	
%	Note that the only words potentially accepted by all automata in the sequence of automata $(A_{c_i})_{c_i \in C}$, $A_\leq n$ are of length \emph{exactly} $n$. Further, note that each $A_{c_i}$ only accepts words of length \emph{exactly} $n$ if they cause the automaton to take a shortcut of the form $\delta_i(q_i^j, \sigma) = q_i^{j+n}$ after a sub-string of length \emph{exactly} $j$ was read. If the transition $\delta_i(q_i^j, \sigma) = q_i^{j+n}$ is taken after a sub-string of length $>j$ was read (i.e., if some self-loop was taken), then the remaining $n-j-1$ letter will not suffice to map the state $q_i^{j+n}$ to the single accepting state~$q_i^{2n-1}$.
%	
%	 
%	 As those transitions where defined only for satisfying assignments for the considered clause, a word accepted by all automata $(A_{c_i})_{c_i \in C}$, $A_\leq n$, encodes a variable assignment satisfying all clauses. Further, an encoding of a satisfying complete variable assignment for the formula $\varphi$ is of length $n$ and causes all automata $A_{c_i}$ to take a shortcut and is hence accepted by all considered automata.
\end{proof}
\todo[inline]{End of toappendix}






%\begin{proof}[Proof of Theorem~\ref{thm:ST-1-NP-hard}]
%	Let $\varphi$ be a Boolean formula in 3-CNF with set of variables $V = \{x_1, x_2, \dots, x_n\}$ and set of clauses $C=\{c_1, c_2, \dots, c_m\}$. From $\varphi$, we construct $m+1$ DFAs over the common alphabet $\Sigma=\{0,1\}$. The input string for these automata will correspond to a variable assignment, therefore, we assume a linear order on $V$ indicated by the indices of the variables. 	
%	
%	For every clause $c_i\in C$, we construct an NFA $A_{c_i}$ consisting of a two phased chain of length $2n$ as $A_{c_i} = (\{\,q_i^j \mid 0 \leq j \leq 2n-1\,\}, \Sigma, \delta_i, q_i^0, \{q_i^{2n-1}\})$. The first $n$ states correspond to the sequence of variables and a read variable assignment that satisfies $c_i$ will cause the automaton to bypass the rest of the states in this part and jump to the corresponding part of the second half of the chain. There, only one state is accepting namely the state that we reach after reading an assignment of exactly $n$ variables which satisfies the clause $c_i$. 
%	To be more formal, for $j \leq n-1$, we define $\delta_i(q_i^j, 0) = q_i^{j+n}$ if $\neg x_{j+1} \in c_i$,  $\delta_i(q_i^j, 1) = q_i^{j+n}$ if $x_{j+1} \in c_i$, and  $\delta_i(q_i^j, \sigma) = q_i^{j+1}$ otherwise, for $\sigma\in \Sigma$ that does not fall under the two previous cases. We further define $\delta_i(q_i^j, \sigma) = q_i^{j+1}$ for $n\leq j < 2n-1$ and $\sigma\in \Sigma$.
%	%	, as well as $\delta_i(q_i^{2n-1}, \sigma) = q_i^{2n-1}$. 
%	So far, $A_{c_i}$ accepts a finite language where all words are of size at least $n$. In order to integrate the accepted language of $A_{c_i}$ into $\st{1/2}$ we add a self-loop, labeled with $\Sigma$, to each state of $A_{c_i}$, i.e., we add the transitions $\delta(q_i^j, \sigma) = q_i^j$ for all $\sigma \in \Sigma$, $0 \leq j \leq 2n-1$.
%	Note that words which correctly encode a complete variable assignment for $V$ are of size exactly $n$. Hence, in order to forbid $A_{c_i}$ to take any of the introduced self-loops, we add a DFA $A_{\leq n}$ that accepts all words of length at most $n$ to the sequence of automata in the intersection. Note that $L(A_{\leq n})$ is the complement of an $\st{1/2}$ language being defined as the finite union $\bigcup_{\sigma_\ell \in \Sigma, \ell \leq n+1} \Sigma^* \sigma_1 \Sigma^* \sigma_2 \dots \sigma_{n+1} \Sigma^*$. 
%	Hence, $L(A_{\leq n})$ is a language from $\st{1}$.
%	For the sake of completeness we construct $A_{\leq n}$ as $A_{\leq n} = (\{q_0, q_1, \dots, q_{n+1}\}, \Sigma, \delta, q_0, \{q_0, q_1, \dots, q_n\})$ with $\delta(q_\ell, \sigma) = q_{\ell+1}$ for $\sigma\in\Sigma$ and $0 \leq \ell \leq n$; and $\delta(q_{n+1}, \sigma) = q_{n+1}$ for $\sigma \in \Sigma$.
%	
%	Note that the only words potentially accepted by all automata in the sequence of automata $(A_{c_i})_{c_i \in C}$, $A_\leq n$ are of length \emph{exactly} $n$. Further, note that each $A_{c_i}$ only accepts words of length \emph{exactly} $n$ if they cause the automaton to take a shortcut of the form $\delta_i(q_i^j, \sigma) = q_i^{j+n}$ after a sub-string of length \emph{exactly} $j$ was read. If the transition $\delta_i(q_i^j, \sigma) = q_i^{j+n}$ is taken after a sub-string of length $>j$ was read (i.e., if some self-loop was taken), then the remaining $n-j-1$ letter will not suffice to map the state $q_i^{j+n}$ to the single accepting state~$q_i^{2n-1}$.
%	
%	As those transitions where defined only for satisfying assignments for the considered clause, a word accepted by all automata $(A_{c_i})_{c_i \in C}$, $A_\leq n$, encodes a variable assignment satisfying all clauses. Further, an encoding of a satisfying complete variable assignment for the formula $\varphi$ is of length $n$ and causes all automata $A_{c_i}$ to take a shortcut and is hence accepted by all considered automata.
%\end{proof}


%In the above construction, the accepting trap states could be replaced by a sequence of $n$ accepting states followed by a rejecting trap state. In this setting, all automata would accept finite languages and hence all accepted languages lie in $\dd{0}$.
%\begin{corollary}\label{cor:DD-0-NP-hard}
%	The \textsc{Intersection Non-Emptiness Problem} for DFAs all accepting languages
%	from~$\dd{0}$ %or $\ddp{0}$ 
%is \NP-hard.
%\end{corollary}
%\begin{remark}
%	In the above construction, the hardness of the \INE problem came from the fact that we could compress the finite languages in a compact form, i.e., every DFA accepts a finite language of size exponential in the size of its state set.
%\end{remark}


%For the level~$\dd{0}$ the following completeness result holds:


%\todo[inline,color=gray!27]{Membership for partially ordered automata (so promise on automata class) is considered in~\cite[Proposition 9]{DBLP:journals/tcs/Ryzhikov19a}.}
%\begin{remark}
%	The \textsc{Intersection Non-emptiness Problem} for automata
%	with the property of being partially ordered has been shown to be \NP-complete in~\cite[Proposition 9]{DBLP:journals/tcs/Ryzhikov19a}.
%\end{remark}

%Let's switch to the first non-trivial full level of the Straubing-Th{\'e}rien hiearchy.
%We can adapt the construction given in Theorem~\ref{thm:DD-1/2-NP-hard} for the \textsc{Intersection Non-emptiness Problem} for NFAs accepting languages of the class $\st{1}$.
\begin{comment}
By a slide adaption of the construction presented in Lemma~\ref{lem:NP-hard-FiniteLang}, i.e., replacing $A_\text{length}$ by two automata which accept all words of length (1) at least $n$ and (2) at most $n$ (language from~$\st{1}$), and adding self-loops to all states of the clause automata, we get a stronger hardness result for $\st{1}$ accepted by NFAs, than the one obtained by language inclusion $\dd{0} \subseteq \st{1}$.
\begin{theorem}\label{thm:ST-1-NP-hard}
	The \INE problem for NFAs is \NP-hard even if only one NFA accepts a language from $\st{1}$ and all other NFAs accept languages
	from~$\st{1/2}$ and the alphabet is binary.
\end{theorem}
\todo[inline]{This proof goes to the appendix}
\begin{proof}
	We adapt the construction given in the proof of Lemma~\ref{lem:NP-hard-FiniteLang} in the following way. 
	We replace the automaton $A_\text{length}$ by two automata $A_{\geq n}$ and $A_{\leq n}$.
	The automaton $A_{\geq n} = (\{q_0, q_1, \dots, q_n\}, \Sigma, \delta, q_0, \{q_n\})$ accepts all words of length at least $n$. More formally, the transition function $\delta$ of $A_{\geq n}$ is defined as $\delta(q_i, \sigma) = q_{i+1}$ for $0 \leq i < n$ and $\delta(q_n, \sigma) = q_n$, for all $\sigma \in \Sigma$. Clearly, $A_{\geq n}$ is a DFA and accepts a co-finite language that is of level $\st{1/2}$.
	
	Consider the automaton $A_{\geq n+1}$ which is similar to $A_{\geq n}$ with the difference that $A_{\geq n+1}$ accepts all words of size at least $n+1$.
	Also $A_{\geq n+1}$ is a DFA accepting a language from level~$\st{1/2}$.
	We now obtain the automaton $A_{\leq n}$ as the complement of $A_{\geq n+1}$, i.e., we replace the set of final states of $A_{\geq n+1}$ by its complement with respect to $Q$. The DFA $A_{\leq n}$ accepts a language from $\st{1}$ as it accepts the complement of a language from $\st{1/2}$.
	Note that, the only words accepted by both $A_{\leq n}$ and $A_{\geq n}$ are of length exactly $n$.
%	 
%	For the automaton $A_\text{length}$ we enrich the set of accepting states to $\{\,q_i \mid i \leq n\,\}$, i.e., we now accept with $A_\text{length}$ all strings of length up to $n$, which is the complement of the language of all strings of length at least $n+1$ which can be expressed in form of a language from $\st{1/2}$, %and $\sts{1/2}$, 
%consisting of a finite union of languages of the form $\Sigma^*\sigma_1\Sigma^*\sigma_2 \Sigma^* \dots \sigma_{n+1}\Sigma^*$ with $\sigma_i \in \Sigma=\{0,1\}$.
%	In order to keep considering only words of length precisely $n$ for candidates of the intersection, we add a new automaton $A_{\text{min }n} = (\{q_\text{min}^0, q_\text{min}^1, \dots, q_\text{min}^n\}, \Sigma, \delta_\text{min}, q_\text{min}^0, \{q_\text{min}^n\})$ with $\delta_\text{min}(q_\text{min}^i, \sigma) = q_\text{min}^{i+1}$ for $i <n$, and $\delta_\text{min}(q_\text{min}^{n}, \sigma) = q_\text{min}^n$ for $\sigma \in \Sigma$. Note that the language of $A_{\text{min }n}$ is the finite union of the languages $\Sigma^*\sigma_1\Sigma^*\sigma_2 \Sigma^* \dots \sigma_{n}\Sigma^*$ over $\sigma_i \in \Sigma=\{0,1\}$.
%	
	Now we adapt the ``clause'' automata $A_{c_i}$ for $c_i \in C$, such that they accept a language of $\st{1/2}$. This adaption will turn the DFAs into NFAs. Therefore, we add in each automata $A_{c_i}$, a non-deterministic self-loop with every letter to each state $q_i^j$, for $0 \leq j \leq 2n$.
	
%	 and roll out the accepting trap state to a sequence of rejecting states followed by one accepting state. The idea of this enrollment is to keep track of from which state we took a shortcut and how many letters we should have to read from this state in order to accept a word of length $n$. Thus, we cannot `hide' in the self-loop of one state in order to shift the meaning of the variable assignment string for some automaton.
	%
%	Hence, we redefine the automata $A_{c_i}$ by $A_{c_i} = (\{\,q_i^j \mid 0 \leq j \leq 2n-1\,\}, \Sigma, \delta_i, q_i^0, \{q_i^{2n-1}\})$ with $\delta_i(q_i^j, \sigma) = q_i^j$ for $j \leq 2n-1$, $\delta_i(q_i^j, \sigma) = q_i^{j+1}$ for $n\leq j \leq 2n-1$ and $\sigma\in \Sigma$. 
%	Further, for $j \leq n-1$, we define $\delta_i(q_i^j, 0) = q_i^{j+n}$ if $\neg x_{j+1} \in c_i$,  $\delta_i(q_i^j, 1) = q_i^{j+n}$ if $x_{j+1} \in c_i$, and  $\delta_i(q_i^j, \sigma) = q_i^{j+1}$ otherwise for $\sigma\in \Sigma$ that does not fall under the two previous cases. Clearly, $L(A_{c_i})$ is of the demanded form for $\st{1/2}$. %and $\sts{1/2}$. 
Note that each $A_{c_i}$ only accepts words of length \emph{exactly} $n$ if they cause the automaton to take a shortcut of the form $\delta_i(q_i^j, \sigma) = q_i^{j+n}$ after a sub-string of length \emph{exactly} $j$ was read. If the transition $\delta_i(q_i^j, \sigma) = q_i^{j+n}$ is taken after a sub-string of length $>j$ was read, then the remaining $n-j-1$ letter will not suffice to map the state $q_i^{j+n}$ to the single accepting state~$q_i^{2n-1}$.
%
%The latter condition ensures that the automaton is still synchronous with the ordering of the variables encoded in the input string and the former condition ensures that the clause is satisfied by the encoded assignment. 
Hence, the words in the intersection of all automata $A_{\leq n}$, $A_{\geq n}$, and $A_{c_i}$ for $c_i \in C$, are precisely the encoded satisfying complete variable assignments for the input formula~$\varphi$.	 
\end{proof}
%\begin{remark}
%	In the construction above, the only automaton accepting a language from $\st{1}\backslash \st{1/2}$ is $A_\text{length}$ accepting the language of all strings of length \emph{up to} $n$. All other automata accepted languages from $\st{1/2}$. 
%\end{remark}\todo{integrate in the proof}
%\todo[inline,color=gray!27]{PW: Again, how do we show membership? We could adapt the argument given in~\cite{DBLP:journals/tcs/Ryzhikov19a} (which is basically our marbles argument) for NFAs, but this is only possible in the setting of automata promises.
%$\Rightarrow$ does LF's comment help here?}
%\todo[color=gray!27,inline]{PW: How expensive is it to make these automata in Theorem~\ref{thm:ST-1-NP-hard} deterministic?}
%\textcolor{blue}{ LF: Probably already follows from the results in the previous section. Confirm.}
%\todo[inline]{HF: I commented my email as this is covered by what is written above, plus \cite{DBLP:journals/corr/abs-1907-13115}.}
\end{comment}
%
\begin{comment}
{\scriptsize
%\begin{verbatim} 
From Henning: Let me be more precise:

As I understood these notions, we could think of level-1 of ST being 
given by "partially ordered confluent DFAs", where "partially ordered" 
is elsewhere named "weakly acyclic".

Then, I think that their constructions prove that non-emptiness of 
intersection of such automata is NP-complete when restricted to 
input alphabets of fixed size (of at least two).

More precisely, if you look at the proof of Lemma 22 in the IC 
paper that I sent around, then in particular Fig. 2 reveals that 
this is "nothing else" than the Eilenberg/Rystsov construction for 
proving NP-hardness of the bounded synchronizing word problem, 
apart from complementation.

To be more explicit, if $(X,C)$ defines an instance of SAT, with 
$X=\{x_1,\dots,x_n\}$, then for each clause $c\in C$, design an 
automaton $A_c$ that only accepts sequences from $\{0,1\}^*$ that 
are either of length $\leq n$ and can be interpreted as an 
assignment satisfying $c$, or are of length $>n$. Moreover, there 
is an automaton accepting all binary strings of length $n$.
All these automata are "partially ordered confluent DFAs".
There is a string accepted by all these automata iff $(X,C)$ is 
satisfiable.

Conversely, membership in NP follows by converting a given bunch 
of "partially ordered confluent DFAs" into one rpoNFA by adding 
a third letter, say 2, to the alphabet and branching with a 2-arc 
from a fresh initial state (where 0,1 loop) into all previous 
initial states and adding 2-arcs from all states of each DFA to a 
"larger" accepting state. (Here, details might be a bit different, 
I did not think about it too much.) After "complementing" accepting 
states of the original DFAs, we should find an instance of rpoNFA 
non-universality that is equivalent to  the non-emptiness-of-intersection 
problem we started with.

Of course, the polynomial length bound on witnesses for all this 
(see Lemma 15 in the IC paper) is crucial here.

I suppose that we can have a similar exploit for level 3/2 of ST 
towards PSPACE-completeness, which altogether would settle our problems.

(OK, we could also look once more on level 1/2 ...)

Best regards, "see" you tomorrow,
Henning
%\end{verbatim}
}
\end{comment}

%\paragraph{\bf Level $3/2$ of STH.}
\subsection{\NP-Membership}
\label{sec:NP-membership}
Next, we focus on the \NP-membership part of \autoref{thm:NPCompleteness} and begin by proving that for~$\dd{0}$, regardless of whether the input automata are NFAs or DFAs, the \INE problem is contained in \NP\ and therefore \NP-complete in combination with~\autoref{NPHardnessBZero}.

%\begin{theorem}\label{thm:DD-0-NPc}
%  The \textsc{Intersection Non-Emptiness Problem} for DFAs or NFAs all accepting languages from~$\dd{0}$ is \NP-complete.
%\end{theorem}
\begin{lemma}\label{thm:DD-0-NPc}
	The \INE problem for DFAs or NFAs all accepting languages from~$\dd{0}$ is contained in \NP.
\end{lemma}
\begin{proof}
	%It remains to show containment in \NP, since the NP-hardness is already shown in Corollary~\ref{cor:DD-0-NP-hard}.
	%
	Let $A_1,A_2,\ldots,A_m$ be an input instance to the \INE problem, where all devices are NFAs accepting languages from $\dd{0}$. If all NFAs accept co-finite languages, which can be verified in deterministic polynomial time, the intersection $\bigcap_{i=1}^m L(A_i)$ is non-empty. Otherwise, there is at least one NFA accepting a finite language, where the longest word is bounded by the number of states of this device. Hence, if $\bigcap_{i=1}^m L(A_i)\neq\emptyset$, there is a word of length polynomial in the length of the input that witnesses this fact. Therefore, such a~$w$ can be nondeterministically guessed by a Turing machine checking membership of~$w$ in~$L(A_i)$, for all NFAs~$A_i$, in sequence. This shows containment in \NP\ as desired.
\end{proof}

Notice that Masopust and Kr\"otzsch have shown in \cite{DBLP:journals/corr/abs-1907-13115}  that \INE for poDFAs and for poNFAs is \NP-complete. Also the unary case is discussed there, which can be solved in polynomial time. We cannot directly make use of these results, as we consider arbitrary NFAs or DFAs as inputs, only with the promise that they accept languages from a certain level of the studied hierarchies.


In order to prove that for the levels $\dd{0}$,\ $\dd{1/2}$,\ $\st{1}$, and~$\st{3/2}$, the \INE problem for DFAs is contained in \NP, it is sufficient to prove the claim for $\st{3/2}$ as all other stated levels are contained in $\st{3/2}$. We prove the latter statement by obtaining a length bound on the length of a shortest word accepted by all DFAs of length polynomial in the size of the biggest DFA\@.\todo{EA: This sentence seems odd to me.} Therefore, we show that for a minimal poNFA $A$, the size of an equivalent DFA is lower-bounded by the size of~$A$ and use a result of Masopust and Kr\"otzsch~\cite{DBLP:journals/corr/abs-1907-13115} for poNFAs.
%Masopust and Kr\"otzsch have shown 
They have shown 
that given poNFAs, $A_1,A_2,\ldots,A_m$,
if the intersection of those poNFAs is non-empty, then there exists a word of size at most
$\sum_{i\in\{1,\ldots,m\}}d_i$,
where $d_i$ is the \emph{depth} of $A_i$ (\cite[Theorem~3.3]{DBLP:journals/corr/abs-1907-13115}).
%We say that a poNFA $A$ is of \emph{depth} $d$
Here, the depth of $A_i$ is the length of the longest path (without self-loops) in the state
graph of $A_i$.
% starting from an initial state. is of length $d$.

This result implies that the \INE problem for poNFAs accepting languages from $\st{3/2}$ is contained in \NP. 
We will further use this
result to show that the \INE problem for DFAs accepting languages from $\st{3/2}$ is \NP-complete.
%\begin{lemma}
%  The \textsc{Intersection Non-emptiness problem} for poNFAs accepting
%  languages from~$\st{3/2}$ belongs to \NP.
%\end{lemma}
%\begin{proof}
%    Let $A_1,A_2,\ldots,A_n$ be an input instance to the intersection non-emptiness problem,
%    where all automata are poNFAs. Suppose that $\cap_{i\in\{1,\ldots,n\}}L(A_i) \neq \emptyset$.
%    Let $w \in \cap_{i\in\{1,\ldots,n\}}L(A_i)$. Let $k_i$ be the number of states in $A_i$.
%    For each $i \in \{1,\ldots,n\}$, we mark letter in $w$ that make $A_i$ change state when
%    reading $w$. $A_i$ is partially ordered, so we mark at most $k_i$ letters. In $w$,
%    there is at most $\sum_{i\in\{1,\ldots,n\}}k_i$ marked letters. Each unmarked letter in $w$
%    correspond to loop in all $A_i$. Let $w'$ be the word obtain from $w$ after
%    removing all unmarked letters. We have that $|w'| \leq \sum_{i\in\{1,\ldots,n\}}k_i$
%    and $w' \in \cap_{i\in\{1,\ldots,n\}}L(A_i)$. Thus if the intersection is not empty,
%    there is a certificate of polynomial size.
%\end{proof}
First, we show that the number of states in a minimal poNFA is at most the number of classes in
the Myhill-Nerode equivalence relation.
Let $A = (Q, \Sigma, \delta, q_0, F)$ be a NFA\@. For each state $q \in Q$, we define
${}_{q}A$ as the automaton obtained from $A$ by replacing the initial state of $A$ by $q$.\todo{HF: We need something similar elsewhere. Should we unify notations for changing initial / final states?}
Therefore, $L({}_{q}A)$ is the language accepted from $q$. More formally,
$L({}_{q}A) = \{\,w \in \Sigma^{*} \mid F \cap \delta(q,w) \neq \emptyset\,\}$. Note that
there is a one-to-one correspondence between $L({}_{q}A)$ and classes in the Myhill-Nerode
equivalence relation.

\begin{theorem}%
    \label{boundSizepoNFA}
    Let $A = (Q, \Sigma, \delta, q_0, F)$ be a minimal poNFA\@. Then, $L({}_{q_1}A) \neq L({}_{q_2}A)$ for all states
    $q_1, q_2 \in Q$.
\end{theorem}
\begin{proof}
	Let $A = (Q, \Sigma, \delta, q_0, F)$  be a minimal poNFA and $q_1, q_2 \in Q$
    be two states. Suppose that $L({}_{q_1}A) = L({}_{q_2}A)$. We have two cases.
	\begin{itemize}
		\item If $q_1$ and $q_2$ are pairwise not reachable from each other, then
		      let $A' = (Q', \Sigma, \delta', q_0, F')$ be the NFA obtained from~$A$, where $q_1$ and~$q_2$
		      are merged into a new state~$q_{1,2}$, so that  $Q' = (Q\setminus\{q_1, q_2\}) \cup \{q_{1,2}\}$,\
		      $\delta'(q_{1,2}, a) = \delta'(q_1, a)
			      \cup \delta'(q_2, a)$, and $q_{1,2} \in F'$ if and only if $q_1 \in F$ or
		      $q_2 \in F$. Automata~$A'$ is a partially ordered NFA\@. As $q_1$ and~$q_2$ are not reachable
		      one from the other, they are incomparable in the partial order relation defined by~$A$. Therefore, there is no state $q$ such that $q_1 < q$ and $q < q_2$. One can check
		      that $L(A') = L(A)$, which contradicts the minimality of~$A$.
		\item Otherwise, $q_1$ is reachable from~$q_2$, or $q_2$ is reachable from~$q_1$.
		      Without loss of generality, we assume that $q_2$ is reachable from~$q_1$.
		      Let $A' = (Q', \Sigma, \delta', q_0, F')$ be the NFA obtained from~$A$ in two steps as described next.
		      First, we remove all outgoing transitions from $q_1$ and then we merge $q_1$ and~$q_2$
		      into a new state $q_{1,2}$ as done before. After removing all outgoing
		      transitions from~$q_1$, $q_2$ is no longer reachable from $q_1$, therefore,
		      as before, $A'$ is a partially ordered NFA\@. Now we will prove that $L(A) = L(A')$.
		      \begin{itemize}
			      \item Let~$w \in L(A)$. Let $\rho$ be an accepting run in $A$.
			            If~$\rho$ does not contain~$q_1$, then the run obtained by replacing every~$q_2$ by~$q_{1,2}$ is an accepting run in~$A'$.
			            If~$\rho$ contains~$q_1$, then we
			            split $w$ into $w_1$ and $w_2$ such that $w = w_1w_2$ and $w_1$ is the shortest
			            prefix of~$w$ such that, after reading~$w_1$, we reach $q_1$ in $\rho$.
			            Because we merged~$q_1$ and~$q_2$ into~$q_{1,2}$, we have that
                        $q_{1,2} \in \delta'(q_0, w_1)$ in~$A'$. Because $L({}_{q_1}A) = L({}_{q_2}A)$, we
                        have that $L({}_{q_1}A) = L({}_{q_2}A) = L({}_{q_{1,2}}A')$ and therefore
			            $\delta'(q_{1,2}, w_2) \cap F' \neq \emptyset$. So, $w$ is accepted by~$A'$.
			      \item Let $w \in L(A')$. Let $\rho$ be an accepting run in $A'$.
			            If $\rho$ does not contain $q_{1,2}$, then the same run is accepting in~$A$, too.
			            If $\rho$ contains $q_{1,2}$, we split $w$ into $w_1$ and~$w_2$  such
			            that $w = w_1w_2$, where $w_1$ is the shortest
			            prefix of $w$ such that, after reading~$w_1$, we reach $q_{1,2}$ in~$\rho$.
                        Then, by definition of $q_{1,2}$, $\delta(q_0, w_1) \cap \{q_1, q_2\} \neq \emptyset$,
                        and $\delta(q_1, w_2) \cap F \neq \emptyset \Leftrightarrow \delta(q_2, w_2) \cap F \neq
                        \emptyset \Leftrightarrow \delta'(q_{1,2}, w_2) \neq \emptyset$.
                        Therefore, $w \in L(A)$.
		      \end{itemize}
              This contradicts the minimality of $A$.
              \qedhere
	\end{itemize}
\end{proof}
\todo[inline]{Add some text for next Lemma}
Now, we can use the result from Masopust and Kr\"otzsch to prove that the \INE{} problem
for DFAs accepting languages in $\st{3/2}$ is in \NP\@.
\begin{lemma}%
  \label{lemma:ST-3/2-DFA}
  The \INE{} problem for DFAs accepting
  languages from~$\st{3/2}$ belongs to \NP\@.
\end{lemma}
\begin{proof}
    By Theorem~\ref{boundSizepoNFA}, we have that the number of state in a minimal
    poNFA is at most the number of class in the Myhill-Nerode equivalence relation.
    Therefore, given a DFA accepting a language from $\st{3/2}$, there exist a smaller
    poNFA that recognises the same language. Therefore, using the result from %Masopust and Kr\"otzsch
    \cite[Theorem~3.3]{DBLP:journals/corr/abs-1907-13115}, if the intersection is not empty, then
    there exists a certificate of polynomial size. Thus the \INE 
    problem for DFAs belongs to \NP\@.
\end{proof}


%\todo[inline]{MO: I think the best is to state Corollary \ref{corollary:NPCompleteness} as a theorem in the 
%beginning of the section. Then we could have 4 subsections, two for the hardness of $\dd{0}$ and $\st{1}$ and 
%two for the easiness of $\dd{1/2}$ and $\st{3/2}$.}

Combining Lemmata~\ref{lem:NP-hard-FiniteLang}\todo{EA: this lemma is no longer in the paper.} and~\ref{lemma:ST-3/2-DFA}, and \cite[Theorem~3.3]{DBLP:journals/corr/abs-1907-13115} with the inclusion
between levels in the Straubing-Th{\'e}rien and the dot-depth hierarchy, we conclude the proof of \autoref{thm:NPCompleteness}.

%have the following result.

%\begin{corollary}
%\label{corollary:NPCompleteness}
%The \textsc{Intersection Non-Emptiness Problem} for DFAs accepting languages from $\dd{0}$,\ $\dd{1/2}$,\ $\st{1}$, or~$\st{3/2}$ is \NP-complete.
%\end{corollary}

%\input{ST3-2-Exchange-Lemma}


\subsection{The Case of Commutative Languages in $\st{3/2}$}

\input{commutative2}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "sample.tex"
%%% End: 



==> LocallyTestableLanguages.tex <==
\todo[inline]{HF / SH: If locally testable languages are re-introduced, we should discuss \cite{Arfi87,Arfi91,zalcstein1972locally}.
\begin{lemma} Normal form: finite union of level $1/2$ with a single complementation
 in each part.
\end{lemma}
}

\section{Locally Testable Languages}



Next, we define the notion of locally testable language according to the terminology 
employed in \cite{zalcstein1972locally}. 

Let $k$ be a positive integer and $w\in \Sigma^+$ be a string of length
at least $k$, we let $L_k(w)$ be the prefix of $w$, $R_k(w)$ be the 
suffix of $w$ and $I_k(w)$ be the set of interior subwords of w of length
$k$. A language $L\subseteq \Sigma^*$ is {\em strictly $k$-testable} if there
are finite test sets $X,Y,Z$ of words over $\Sigma$  such that for all
$w\in \Sigma^+$, $|w|\geq k$, $w\in L$ if and only if $L_k(w)\in X$, $R_k(w)\in Y$
and $I_{k}(w)\subseteq Z$. $L$ is strictly locally testable if it is strictly
locally testable for some $k>0$. 


A language $L\in \Sigma^+$ is $k$-testable if $L$ is a Boolean combination of 
strictly $k$-testable languages. $L$ is locally testable if it is $k$-testable 
for some $k>0$. 

\todo{SH: Isn't this only the case of strictly $k$-testable?}
\begin{lemma}
	Let $L_1,\dots,L_n$ be $k$-testable languages over an alphabet $\Sigma$ with test sets 
	$(X_1,Y_1,Z_1)\dots (X_n,Y_n,Z_n)$ respectively. Then, emptiness of intersection can
	be decided in time $O(|\Sigma|^r\cdot n)$.\todo[color=gray!27]{PW:Don't you mean $k$ instead of $r$ here?}
\end{lemma}
\begin{proof}
	\begin{enumerate}
		\item Let $r$ be the largest size of a string in some of the test sets. 
		\item For each $i\in [n]$, construct a new test set $(X_i',Y_i',Z_i')$
			characterizing  the languages $L_i$ with the property that each 
			string in each of the three sets has size $r$.
		\item Note that an upper bound for the size or each set is $|\Sigma|^r$. Therefore,
			all triples  $(X_i',Y_i',Z_i')$ can be constructed in time $O(|\Sigma|^r\cdot n)$.
		\item Now let $X = \bigcap_{i\in [n]} X_i'$, $Y= \bigcap_{i\in[n]} Y_i'$
			and $Z = \bigcap_{i\in [n]} Z_i'$. We claim that $(X,Y,Z)$ characterizes
			$\bigcap_{i} L_i$. Note that the triple $(X,Y,Z)$ can be constructed in time $O(|\Sigma|^{r}\cdot n)$. 
		\item Finally, we test whether the language characterized by $(X,Y,Z)$ is non-empty. 
			Towards this goal, we create an automaton $A$ whose states are the strings in $\{q_0\}\cup X\cup Y \cup Z$, 
			$q_0$ is the unique initial state, the final statse are the strings in $Z$, and the transition relation
			is $\Delta = \{(q_0,u,u)\;|\; u\in X\}\cup \{(au,b,ub)\;|\; a\in \Sigma, ub\in Y \} \cup \{(au,b,ub)\;|\; ub\in Z\}$. 
			We claim that $L$ is the language of $A$. \textcolor{red}{Obs: in the first set, the transitions read strings instead of symbols.}
		\item Determining whether the language generated by $A$ is non-empty can be done in NL using standard reachability algorithms. 
			It can also be solved in time $O(|\Sigma|^k\cdot n)$ time using space $|\Sigma|^k\cdot n$. 
	\end{enumerate}
\end{proof}



\newpage




==> TransformationMonoidMembership.tex <==
\section{Intersection non-emptiness and transformation monoid membership}

{\color{blue}
  LF: First very rough draft; proofs are only sketches. Proofs need to be
  checked and polished, notation needs to be unified, many definitions missing.
  Intersection non-emptiness problem for a (pseudo-)variety here refers to the
  DFA variant with transition monoids of all DFAs belonging to a given variety.
}

\begin{theorem}
  The transformation monoid membership problem for a variety $\mathbf{V}$ of
  finite monoids is reducible to the intersection non-emptiness problem of
  $\mathbf{V}$ under log-space reductions.
\end{theorem}
%
\begin{proof}
  Let $Q$ be a finite set and let $a_1, \dots, a_m, t \colon Q \to Q$ be a set
  of transformations on a common set $Q$.\todo[color=gray!27]{MH: please $a_1,a_2,\ldots,a_m$ instead of $a_1,\ldots, a_m$.}
  %
  Define a family of automata $\{A_q\}_{q \in Q}$, each with the same set of
  states $Q$ and the same set of transitions, induced by $a_1, \dots, a_m$. For
  each $q \in Q$, the initial state of the automaton $A_q$ is $q$ and the only
  final state is $t(q)$.
  %
  By construction, $t$ belongs to the transformation monoid generated by $a_1,
  \dots, a_m$ if and only if $L(A_1) \cap \cdots \cap L(A_n)$ is non-empty. \todo[color=gray!27]{MH: I would prefer $\bigcap_{q\in Q} L(A_q)$} The
  transition monoid of each automaton $A_q$ is isomorphic to the monoid
  generated by $a_1, \dots, a_m$ and thus belongs to $\mathbf{V}$.
\end{proof}

\begin{theorem}
  The intersection non-emptiness problem for a variety $\mathbf{V}$ of finite
  monoids is $\NP$-reducible\todo[color=gray!27]{MH: is NL many-one reducibility enough?} to the transformation monoid membership problem
  of~$\mathbf{V}$.
\end{theorem}
%
\begin{proof}
  We first reduce intersection non-emptiness to the transformation monoid
  membership problem. Let $A_1, \dots, A_n$ be a set of DFA with state sets
  $Q_1, \dots, Q_n$, initial states $q_1, \dots, q_n$ and final states $F_1,
  \dots, F_n$ respectively.
  %
  To simplify notation, let $Q = Q_1 \cup \cdots \cup Q_n$ and $F = F_1 \cup
  \cdots \cup F_n$.
  %
  Without loss of generality, we assume that all automata use a common alphabet
  $\Sigma$ and we identify each letter $a \in \Sigma$ with the action $a \colon
  Q \to Q$ of the letter on the set of states.

  We guess a mapping $t \colon Q \to Q$ (by guessing a state $t(q)$ for each $q
  \in Q$) and check that $t(q_i) \in F$ for all $i \in \{1, \dots, n\}$.
  %
  The resulting transformation monoid membership instance is comprised of the
  transformations $a \colon Q \to Q$ for all $a \in \Sigma$ and $t \colon Q \to
  Q$.
  %
  It is easy to see that $t$ belongs to the transformation monoid generated by
  the transformations in $\Sigma$ if and only if $L(A_1) \cap \cdots \cap
  L(A_n)$ is non-empty.
  %
  The transformation monoid divides the direct product of the transition
  monoids of $A_1, \dots, A_n$ and therefore belongs to $\mathbf{V}$.
\end{proof}

Together with results from ``Membership Testing in Commutative Transformation
Semigroups'' and ``The Membership Problem in Aperiodic Transformation
Monoids'' we obtain the following corollary.
%
{\color{blue}LF: Add proper citations.}

\begin{corollary}
  The intersection non-emptiness problem is $\NP$-complete for the varieties
  $\mathbf{R}$, $\mathbf{B}$, $\mathbf{Acom}$ and $\mathbf{Com}$.
\end{corollary}

{\color{blue}
  LF: Corollary incomplete. These are the most interesting cases but more
  results follow from the papers cited in the paragraph above.
  %
  \begin{itemize}
    \item $\mathbf{R}$ is $\mathcal{R}$-trivial
    \item $\mathbf{B}$ is idempotent.
    \item $\mathbf{Acom}$ is aperiodic commutative.
    \item $\mathbf{Com}$ is commutative.
  \end{itemize}
}





==> commutative.tex <==
\section{Commutative Aperiodic Automata}

Here, we show that \textsc{Intersection-Non-Emptiness}
for aperiodic commutative automata is decidable in polynomial time
for \emph{fixed alphabets}, and both for DFAs
and for partially ordered NFAs as input.

In Subsection~\ref{subsec:comm_DFA}, we show it for 
$k$ DFAs, each recognizing a star-free commutative language.
Lastly, in Subsection~\ref{subsec:NEA_com}, we show it for 
$k$ partially ordered NFAs, each recognizing a star-free commutative language.

In the latter case, we also argue that the model of non-deterministic automata
chosen is sufficient to recognize every star-free commutative language.

\subsection{The Case of Deterministic Commutative Automata}
\label{subsec:comm_DFA}

\begin{theorem}
\label{thm:DFA_int_com}
 Let $A_i = (\Sigma, Q_i, \delta_i, q_i, F_i)$, $i \in \{1,\ldots,k\}$,
 be $k$ deterministic automata recognizing commutative and star-free languages.
 Then, the problem if they all accept a common word could be decided
 in polynomial time for a fixed alphabet.
\end{theorem}
\begin{proof}
 By minimizing the input automata, we can assume them to be aperiodic.
 Let $a \in \Sigma$. Set
 \[
  N_a = \max\{ |\{ \delta_i(q_i, a^n) \mid n \ge 0 \}| : i \in \{1,\ldots,k\} \}.
 \]
 By the aperiodicity\footnote{Recall that an automaton is called aperiodic~\cite{McNaughton71}, if no word induces a permutation of some subset of states. We use this in particular for the letters here.} of the automata, we have,
 for any $i \in \{1,\ldots,k\}$, 
 \begin{equation} \label{eqn:C_aperiodic}
     \delta_i(q_i, a^{N_a-1}) = \delta_i(q_i, a^{N_a}).
 \end{equation}
 Fix an order $\Sigma = \{a_1, \ldots, a_m\}$ on the letters.
 Then, we have, for any $i \in \{1,\ldots, k\}$, 
 by commutativity and Equation~\eqref{eqn:C_aperiodic},
 \[
  w \in L( A_i) 
  \Leftrightarrow 
  a_1^{\min\{ N_{a_1}, |w|_{a_1} \}} \cdots a_m^{\min\{ N_{a_m}, |w|_{a_m} \}} \in L(A_i).
 \]
 So,
 \[
  w \in \bigcap_{i=1}^k L(A_i) 
  \Leftrightarrow 
  a_1^{\min\{ N_{a_1}, |w|_{a_1} \}} \cdots a_m^{\min\{ N_{a_m}, |w|_{a_m} \}} \in \bigcap_{i=1}^k L(A_i),
 \]
 which implies that to find out if $\bigcap_{i=1}^k L(A_i) \ne \emptyset$,
 we only have to test the words
 \[
  a_1^{n_1} \cdots a_m^{n_m}
 \]
 with $0 \le n_j < N_{a_j}$ for $j \in \{1,\ldots,m\}$.
 Each test could be run in polynomial time for each automaton, and
 we have to perform at most $N_{a_1} \cdots N_{a_m} \le N^m$ many tests,
 where $N = \max\{ |Q_i| : i \in \{1,\ldots, k\}\}$
 and $m = |\Sigma|$.
\end{proof}




\subsection{The Case of Non-Deterministic Commutative Automata}
\label{subsec:NEA_com}


For a commutative semigroup $S$, we have, for $s, t \in S$,
that $s \mathcal R t$ iff $s \mathcal L t$.
Hence, the $\mathcal R$, $\mathcal L$ and the $\mathcal H$ equivalence
relations coincide.
In particular, the syntactic monoid of a commutative language
is $\mathcal R$-trivial iff it is $\mathcal H$-trivial, i.e., aperiodic.

In general, the class of languages recognized by $\mathcal R$-trivial 
monoids is contained strictly between level $1$ and $3/2$ 
of the Straubing-Th{\'e}rien hierarchy.
In~\cite{DBLP:conf/dlt/SchwentickTV01}, it was shown that the class of
languages recognizable by partially ordered NFAs is precisely
the class of languages at level $3/2$ of the Straubing-Therien-Hierarchy.
The languages recognized by  $\mathcal R$-trivial
monoids are precisely those recognizable by partially ordered DFAs~\cite{DBLP:journals/jcss/BrzozowskiF80}\todo{\cite{DBLP:journals/jcss/BrzozowskiF80}\\
PW: didn't we had a level assigned with poDFAs? \\ SH: No... In general, poDFA languages lie strictly between level one and three-half of the ST-Hierarchy.}.
Hence, we conclude that every commutative aperiodic language
is given by a partially ordered NFA \todo{PW: It should be made clear, that commutative aperiodic languages are a strict sub-class of the class of languages recognized by $\mathcal{R}$-trivial monoids, respectively poDFAs. SH: Done.}, and that, if we have 
some partially ordered NFA recognizing a commutative language, then
it is aperiodic.
So, we conclude that every commutative and aperiodic language could
be given by a partially ordered DFA or NFA. In particular, the commutative aperiodic
languages are a strict subclass of the $\mathcal R$-trivial languages.
In this chapter, we will assume that our language is given by
a partially ordered NFA.

\begin{lemma}
\label{lem:length_of_unary_path_star_free_NEA}
 Let $A = (\Sigma, Q, \delta, q_0, F)$ be a partially ordered NFA
 and\todo{SH: Introduce notation $\delta(S, w) = \{ \delta(q, w) : q \in S \}$
 above.}
 $S \subseteq Q$.
 Then, \[ 
 \delta(S, a^{|Q|}) = \delta(S, a^{|Q|+1}).
 \] 
\end{lemma}
\begin{proof}
    Suppose we have a path, only labeled with $a$, of length $|Q|$.
    Then, this path contains $|Q|+1$ states, i.e., at least
    on state must be repeated.
    As the automaton is partially ordered,
    such a repetition must occur between direct neighbors in the path.
    So, by going one additional round, we have a path
    of length $|Q|+1$ with the same ending state.
    This shows $\delta_P(S, a^{|Q|}) \subseteq \delta_P(S, a^{|Q|+1})$.
    
    Conversely, if we have a path of length $|Q|+1$, we also must have
    a repetition, which could be left out, giving a path of length $|Q|$.
    This shows the other inclusion.
 \end{proof}


 
 Now, we can show that for partially ordered NFAs recognizing
 a commutative language, the problem if they all accept
 a common word could be solved in polynomial time
 for \emph{fixed alphabets}.
 
 \begin{theorem}
  Let $A_i = (\Sigma, Q_i, \delta_i, q_i, F_i)$ for $i \in \{1,\ldots,k\}$
  be $k$ partially ordered NFAs\footnote{We do not assume other conditions than to recognize 
  a commutative language. For example, it is not assumed that, if $q \in \delta(p, ab)$, we must have $q \in \delta(p, ba)$.} 
  such that $L(A_i)$
  is commutative.
  Then, the problem if they all accept a common word
  could be decided in polynomial time for a fixed alphabet.\todo{PW: As stated this is again not polynomial.
  SH: I have added that we suppose a fixed alphabet here.}
 \end{theorem}
 \begin{proof}
  Fix any order $\Sigma = \{a_1,\ldots,a_m\}$
  of the alphabet.
  By commutativity, for $w \in \Sigma^*$ and $i \in \{1,\ldots, k\}$,
  \[
   \delta_i(\{q_0\}, w) \cap F_i \ne \emptyset
   \Leftrightarrow 
   \delta_i(\{q_0\}, a_1^{|w|_{a_1}} \cdots a_m^{|w|_{a_m}}) \cap F_i \ne \emptyset.
  \]
  By Lemma~\ref{lem:length_of_unary_path_star_free_NEA},
  \begin{multline*}
   \delta_i(\{q_0\}, a_1^{|w|_{a_1}} \cdots a_m^{|w|_{a_m}}) \cap F_i \ne \emptyset
   \\ \Leftrightarrow
   \delta_i(\{q_0\}, a_1^{\min\{|Q_i|, |w|_{a_1}\}} \cdots a_m^{\min\{|Q_i|, |w|_{a_m}\}})
   \cap F_i \ne \emptyset
  \end{multline*}
  for each $i \in \{1,\ldots,k\}$.
  Hence, similar as in the proof of Theorem~\ref{thm:DFA_int_com},
  we only have to test the words
  \[
   a_1^{n_1} \cdots a_m^{n_m}
  \]
  with $0 \le n_j < N$ for $j \in \{1,\ldots,m\}$,
  where $N = \max\{ |Q_i| : i \in \{1,\ldots,k\} \}$, 
  giving a polynomial time procedure for a fixed alphabet.
 \end{proof}


==> diagram_commutative.tex <==
\begin{tikzpicture}[>=stealth']
    \def\dist{3}
	\node at (0,0) (st0) {$\st{0}$};
    \path (st0) +(\dist, 2) node (dd0) {$\dd{0}$};
    \path (st0) ++(\dist,0) ++(\dist,0) node (st12) {$\st{\frac{1}{2}} = \dd{\frac{1}{2}}$};
    \path (st12) ++(\dist,0) node (st1) {$\st{1} = \dd{1}$};
    \path (st1) ++(\dist,0) node (st32) {$\st{\frac{3}{2}} = \dd{\frac{3}{2}}$};
    \useasboundingbox (-1,-1) rectangle (13, 3);

	\draw[->] (st0) to (dd0);
	\draw[->] (st0) to (st12);
	\draw[->] (st12) to (st1);
	\draw[->] (st1) to (st32);

	\draw[->] (dd0) to (st12);

	\begin{pgfonlayer}{background}
        \fill[color=yellow!10] (st0) +(-1, 1) .. controls +(90:3) and +(90:4) .. +(13, 0)
            .. controls +(-90:2) and +(-90:3) .. cycle;

		\draw[color=yellow!30,line width=8,line cap=round,name path=nl] (st0) +(-1, 1)
            .. controls +(90:3) and +(90:4) .. node[color=black, near end] [sloped] {\NP} +(13, 0)
            .. controls +(-90:2) and +(-90:3) .. cycle;
        \fill[color=green!10] (st0) +(-.5, 1) to[out=45, in=90] +(7.5, 0) .. controls +(-90:2) and +(-135:3) .. cycle;

		\draw[color=green!30,line width=8,line cap=round,name path=nl] (st0) +(-.5, 1) to[out=45, in=90] node[color=black, midway] [sloped] {\NL} +(7.5, 0) .. controls +(-90:2) and +(-135:3) .. cycle;
        \path[name path=bottom] (st0) ++(1, -0.5) to +(0,-2);
        \path[name intersections={of= nl and bottom }] (intersection-1) node (bottom) {};
        \draw[color=green!30,line width=2,line cap=round,dashed] (st0) +(-.5, 1) to[out=45, in=90] +(1, -0.5) to (bottom);
	\end{pgfonlayer}

\end{tikzpicture}

